RF characterization and beam measurements with 3D printed Fast Faraday Cups

The early stages of most particle accelerator chains produce sub-ns bunches with velocities in the range of 1 to 20% of the speed of light. Fast Faraday Cups (FFC) are designed to measure the longitudinal charge distribution of these short bunches of free charges. Coaxial designs have been utilized at the GSI's linear accelerator UNILAC to characterize ion bunches with bunch lengths ranging from a few hundred ps to a few ns. The typical design goals are to avoid the pre-field of the charges and to suppress secondary electron emission, while retaining the capability of bunch-by-bunch measurements. In this contribution, a novel FFC design manufactured using additive manufacturing, e.g. laser powder bed fusion is presented and compared with a traditionally produced FFC. The design considerations, RF characterization, and selected measurements with ion beam at GSI are shown.

==> Definitions/journalnames.tex <==
% Updated 4 September 2024
%% --------------------------------------------------------------------
%\DeclareOption{}{%
%	\gdef\@journal{}
%	\gdef\@journalfull{}
%	\gdef\@journalshort{}
%	\gdef\@doiabbr{}
%	\gdef\@ISSN{}
%	\gdef\@continuouspages{yes}
%	\gdef\@societyowner{}
%}
%% --------------------------------------------------------------------
%% Fields meanings:
%% - Option name: Journal website name (used in URL)
%% - @journal: Journal website name (used in URL)
%% - @journalfull: Journal full name
%% - @journalshort: Short Name (ISO4)
%% - @doiabbr: DOI abbreviation of the journal used in DOI numbers 10.3390/journalnameXXXX
%% - @ISSN: Journal E-ISSN number
%% - @continuouspages: use \gdef\@continuouspages{yes} for journals that use pagination
%% - @societyowner: Name of society owning the journal (for society journals)
%% --------------------------------------------------------------------
\DeclareOption{acoustics}{%
    \gdef\@journal{acoustics}
    \gdef\@journalfull{Acoustics}
    \gdef\@journalshort{Acoustics}
    \gdef\@doiabbr{acoustics}
    \gdef\@ISSN{2624-599X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{actuators}{%
    \gdef\@journal{actuators}
    \gdef\@journalfull{Actuators}
    \gdef\@journalshort{Actuators}
    \gdef\@doiabbr{act}
    \gdef\@ISSN{2076-0825}
    \gdef\@societyowner{}
}
\DeclareOption{addictions}{%
    \gdef\@journal{addictions}
    \gdef\@journalfull{Addictions}
    \gdef\@journalshort{Addictions}
    \gdef\@doiabbr{addictions}
    \gdef\@ISSN{0006-0006}
    \gdef\@societyowner{}
}
\DeclareOption{adhesives}{%
    \gdef\@journal{adhesives}
    \gdef\@journalfull{Adhesives}
    \gdef\@journalshort{Adhesives}
    \gdef\@doiabbr{adhesives}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{admsci}{%
    \gdef\@journal{admsci}
    \gdef\@journalfull{Administrative Sciences}
    \gdef\@journalshort{Adm. Sci.}
    \gdef\@doiabbr{admsci}
    \gdef\@ISSN{2076-3387}
    \gdef\@societyowner{}
}
\DeclareOption{adolescents}{%
    \gdef\@journal{adolescents}
    \gdef\@journalfull{Adolescents}
    \gdef\@journalshort{Adolescents}
    \gdef\@doiabbr{adolescents}
    \gdef\@ISSN{2673-7051}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{aerobiology}{%
    \gdef\@journal{aerobiology}
    \gdef\@journalfull{Aerobiology}
    \gdef\@journalshort{Aerobiology}
    \gdef\@doiabbr{aerobiology}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{aerospace}{%
    \gdef\@journal{aerospace}
    \gdef\@journalfull{Aerospace}
    \gdef\@journalshort{Aerospace}
    \gdef\@doiabbr{aerospace}
    \gdef\@ISSN{2226-4310}
    \gdef\@societyowner{}
}
\DeclareOption{agriculture}{%
    \gdef\@journal{agriculture}
    \gdef\@journalfull{Agriculture}
    \gdef\@journalshort{Agriculture}
    \gdef\@doiabbr{agriculture}
    \gdef\@ISSN{2077-0472}
    \gdef\@societyowner{}
}
\DeclareOption{agriengineering}{%
    \gdef\@journal{agriengineering}
    \gdef\@journalfull{AgriEngineering}
    \gdef\@journalshort{AgriEngineering}
    \gdef\@doiabbr{agriengineering}
    \gdef\@ISSN{2624-7402}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{agrochemicals}{%
    \gdef\@journal{agrochemicals}
    \gdef\@journalfull{Agrochemicals}
    \gdef\@journalshort{Agrochemicals}
    \gdef\@doiabbr{agrochemicals}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{agronomy}{%
    \gdef\@journal{agronomy}
    \gdef\@journalfull{Agronomy}
    \gdef\@journalshort{Agronomy}
    \gdef\@doiabbr{agronomy}
    \gdef\@ISSN{2073-4395}
    \gdef\@societyowner{}
}
\DeclareOption{ai}{%
    \gdef\@journal{ai}
    \gdef\@journalfull{AI}
    \gdef\@journalshort{AI}
    \gdef\@doiabbr{ai}
    \gdef\@ISSN{2673-2688}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{air}{%
    \gdef\@journal{air}
    \gdef\@journalfull{Air}
    \gdef\@journalshort{Air}
    \gdef\@doiabbr{air}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{algorithms}{%
    \gdef\@journal{algorithms}
    \gdef\@journalfull{Algorithms}
    \gdef\@journalshort{Algorithms}
    \gdef\@doiabbr{a}
    \gdef\@ISSN{1999-4893}
    \gdef\@societyowner{}
}
\DeclareOption{allergies}{%
    \gdef\@journal{allergies}
    \gdef\@journalfull{Allergies}
    \gdef\@journalshort{Allergies}
    \gdef\@doiabbr{allergies}
    \gdef\@ISSN{2313-5786}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{alloys}{%
    \gdef\@journal{alloys}
    \gdef\@journalfull{Alloys}
    \gdef\@journalshort{Alloys}
    \gdef\@doiabbr{alloys}
    \gdef\@ISSN{2674-063X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{amh}{%
    \gdef\@journal{amh}
    \gdef\@journalfull{Acta Microbiologica Hellenica}
    \gdef\@journalshort{Acta Microbiol. Hell.}
    \gdef\@doiabbr{amh}
    \gdef\@ISSN{0438-9573}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{Hellenic Society for Microbiology}
}
\DeclareOption{analytica}{%
    \gdef\@journal{analytica}
    \gdef\@journalfull{Analytica}
    \gdef\@journalshort{Analytica}
    \gdef\@doiabbr{analytica}
    \gdef\@ISSN{2673-4532}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{analytics}{%
    \gdef\@journal{analytics}
    \gdef\@journalfull{Analytics}
    \gdef\@journalshort{Analytics}
    \gdef\@doiabbr{analytics}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{anatomia}{%
    \gdef\@journal{anatomia}
    \gdef\@journalfull{Anatomia}
    \gdef\@journalshort{Anatomia}
    \gdef\@doiabbr{anatomia}
    \gdef\@ISSN{2813-0545}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{anesthres}{%
    \gdef\@journal{anesthres}
    \gdef\@journalfull{Anesthesia Research}
    \gdef\@journalshort{Anesth. Res.}
    \gdef\@doiabbr{anesthres}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{animals}{%
    \gdef\@journal{animals}
    \gdef\@journalfull{Animals}
    \gdef\@journalshort{Animals}
    \gdef\@doiabbr{ani}
    \gdef\@ISSN{2076-2615}
    \gdef\@societyowner{}
}
\DeclareOption{antibiotics}{%
    \gdef\@journal{antibiotics}
    \gdef\@journalfull{Antibiotics}
    \gdef\@journalshort{Antibiotics}
    \gdef\@doiabbr{antibiotics}
    \gdef\@ISSN{2079-6382}
    \gdef\@societyowner{}
}
\DeclareOption{antibodies}{%
    \gdef\@journal{antibodies}
    \gdef\@journalfull{Antibodies}
    \gdef\@journalshort{Antibodies}
    \gdef\@doiabbr{antib}
    \gdef\@ISSN{2073-4468}
    \gdef\@societyowner{}
}
\DeclareOption{antioxidants}{%
    \gdef\@journal{antioxidants}
    \gdef\@journalfull{Antioxidants}
    \gdef\@journalshort{Antioxidants}
    \gdef\@doiabbr{antiox}
    \gdef\@ISSN{2076-3921}
    \gdef\@societyowner{}
}
\DeclareOption{applbiosci}{%
    \gdef\@journal{applbiosci}
    \gdef\@journalfull{Applied Biosciences}
    \gdef\@journalshort{Appl. Biosci.}
    \gdef\@doiabbr{applbiosci}
    \gdef\@ISSN{2813-0464}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{appliedchem}{%
    \gdef\@journal{appliedchem}
    \gdef\@journalfull{AppliedChem}
    \gdef\@journalshort{AppliedChem}
    \gdef\@doiabbr{appliedchem}
    \gdef\@ISSN{2673-9623}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{appliedmath}{%
    \gdef\@journal{appliedmath}
    \gdef\@journalfull{AppliedMath}
    \gdef\@journalshort{AppliedMath}
    \gdef\@doiabbr{appliedmath}
    \gdef\@ISSN{2673-9909}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{appliedphys}{%
    \gdef\@journal{appliedphys}
    \gdef\@journalfull{AppliedPhys}
    \gdef\@journalshort{AppliedPhys}
    \gdef\@doiabbr{appliedphys}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{applmech}{%
    \gdef\@journal{applmech}
    \gdef\@journalfull{Applied Mechanics}
    \gdef\@journalshort{Appl. Mech.}
    \gdef\@doiabbr{applmech}
    \gdef\@ISSN{2673-3161}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{applmicrobiol}{%
    \gdef\@journal{applmicrobiol}
    \gdef\@journalfull{Applied Microbiology}
    \gdef\@journalshort{Appl. Microbiol.}
    \gdef\@doiabbr{applmicrobiol}
    \gdef\@ISSN{2673-8007}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{applnano}{%
    \gdef\@journal{applnano}
    \gdef\@journalfull{Applied Nano}
    \gdef\@journalshort{Appl. Nano}
    \gdef\@doiabbr{applnano}
    \gdef\@ISSN{2673-3501}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{applsci}{%
    \gdef\@journal{applsci}
    \gdef\@journalfull{Applied Sciences}
    \gdef\@journalshort{Appl. Sci.}
    \gdef\@doiabbr{app}
    \gdef\@ISSN{2076-3417}
    \gdef\@societyowner{}
}
\DeclareOption{aquacj}{%
    \gdef\@journal{aquacj}
    \gdef\@journalfull{Aquaculture Journal}
    \gdef\@journalshort{Aquac. J.}
    \gdef\@doiabbr{aquacj}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{architecture}{%
    \gdef\@journal{architecture}
    \gdef\@journalfull{Architecture}
    \gdef\@journalshort{Architecture}
    \gdef\@doiabbr{architecture}
    \gdef\@ISSN{2673-8945}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{arm}{%
    \gdef\@journal{arm}
    \gdef\@journalfull{Advances in Respiratory Medicine}
    \gdef\@journalshort{Adv. Respir. Med.}
    \gdef\@doiabbr{arm}
    \gdef\@ISSN{2543-6031}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{Polish Respiratory Society}
}
\DeclareOption{arthropoda}{%
    \gdef\@journal{arthropoda}
    \gdef\@journalfull{Arthropoda}
    \gdef\@journalshort{Arthropoda}
    \gdef\@doiabbr{arthropoda}
    \gdef\@ISSN{2813-3323}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{arts}{%
    \gdef\@journal{arts}
    \gdef\@journalfull{Arts}
    \gdef\@journalshort{Arts}
    \gdef\@doiabbr{arts}
    \gdef\@ISSN{2076-0752}
    \gdef\@societyowner{}
}
\DeclareOption{asc}{%
    \gdef\@journal{asc}
    \gdef\@journalfull{Automatic Systems and Control}
    \gdef\@journalshort{Autom. Syst. Control}
    \gdef\@doiabbr{}
    \gdef\@ISSN{}
    \gdef\@societyowner{}
}
\DeclareOption{asi}{%
    \gdef\@journal{asi}
    \gdef\@journalfull{Applied System Innovation}
    \gdef\@journalshort{Appl. Syst. Innov.}
    \gdef\@doiabbr{asi}
    \gdef\@ISSN{2571-5577}
    \gdef\@societyowner{International Institute of Knowledge Innovation and Invention}
}
\DeclareOption{astronomy}{%
    \gdef\@journal{astronomy}
    \gdef\@journalfull{Astronomy}
    \gdef\@journalshort{Astronomy}
    \gdef\@doiabbr{astronomy}
    \gdef\@ISSN{2674-0346}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{atmosphere}{%
    \gdef\@journal{atmosphere}
    \gdef\@journalfull{Atmosphere}
    \gdef\@journalshort{Atmosphere}
    \gdef\@doiabbr{atmos}
    \gdef\@ISSN{2073-4433}
    \gdef\@societyowner{}
}
\DeclareOption{atoms}{%
    \gdef\@journal{atoms}
    \gdef\@journalfull{Atoms}
    \gdef\@journalshort{Atoms}
    \gdef\@doiabbr{atoms}
    \gdef\@ISSN{2218-2004}
    \gdef\@societyowner{}
}
\DeclareOption{audiolres}{%
    \gdef\@journal{audiolres}
    \gdef\@journalfull{Audiology Research}
    \gdef\@journalshort{Audiol. Res.}
    \gdef\@doiabbr{audiolres}
    \gdef\@ISSN{2039-4349}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{automation}{%
    \gdef\@journal{automation}
    \gdef\@journalfull{Automation}
    \gdef\@journalshort{Automation}
    \gdef\@doiabbr{automation}
    \gdef\@ISSN{2673-4052}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{axioms}{%
    \gdef\@journal{axioms}
    \gdef\@journalfull{Axioms}
    \gdef\@journalshort{Axioms}
    \gdef\@doiabbr{axioms}
    \gdef\@ISSN{2075-1680}
    \gdef\@societyowner{}
}
\DeclareOption{bacteria}{%
    \gdef\@journal{bacteria}
    \gdef\@journalfull{Bacteria}
    \gdef\@journalshort{Bacteria}
    \gdef\@doiabbr{bacteria}
    \gdef\@ISSN{2674-1334}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{batteries}{%
    \gdef\@journal{batteries}
    \gdef\@journalfull{Batteries}
    \gdef\@journalshort{Batteries}
    \gdef\@doiabbr{batteries}
    \gdef\@ISSN{2313-0105}
    \gdef\@societyowner{}
}
\DeclareOption{bdcc}{%
    \gdef\@journal{bdcc}
    \gdef\@journalfull{Big Data and Cognitive Computing}
    \gdef\@journalshort{Big Data Cogn. Comput.}
    \gdef\@doiabbr{bdcc}
    \gdef\@ISSN{2504-2289}
    \gdef\@societyowner{}
}
\DeclareOption{behavsci}{%
    \gdef\@journal{behavsci}
    \gdef\@journalfull{Behavioral Sciences}
    \gdef\@journalshort{Behav. Sci.}
    \gdef\@doiabbr{bs}
    \gdef\@ISSN{2076-328X}
    \gdef\@societyowner{}
}
\DeclareOption{beverages}{%
    \gdef\@journal{beverages}
    \gdef\@journalfull{Beverages}
    \gdef\@journalshort{Beverages}
    \gdef\@doiabbr{beverages}
    \gdef\@ISSN{2306-5710}
    \gdef\@societyowner{}
}
\DeclareOption{biochem}{%
    \gdef\@journal{biochem}
    \gdef\@journalfull{BioChem}
    \gdef\@journalshort{BioChem}
    \gdef\@doiabbr{biochem}
    \gdef\@ISSN{2673-6411}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{bioengineering}{%
    \gdef\@journal{bioengineering}
    \gdef\@journalfull{Bioengineering}
    \gdef\@journalshort{Bioengineering}
    \gdef\@doiabbr{bioengineering}
    \gdef\@ISSN{2306-5354}
    \gdef\@societyowner{}
}
\DeclareOption{biologics}{%
    \gdef\@journal{biologics}
    \gdef\@journalfull{Biologics}
    \gdef\@journalshort{Biologics}
    \gdef\@doiabbr{biologics}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{biology}{%
    \gdef\@journal{biology}
    \gdef\@journalfull{Biology}
    \gdef\@journalshort{Biology}
    \gdef\@doiabbr{biology}
    \gdef\@ISSN{2079-7737}
    \gdef\@societyowner{}
}
\DeclareOption{biomass}{%
    \gdef\@journal{biomass}
    \gdef\@journalfull{Biomass}
    \gdef\@journalshort{Biomass}
    \gdef\@doiabbr{biomass}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{biomechanics}{%
    \gdef\@journal{biomechanics}
    \gdef\@journalfull{Biomechanics}
    \gdef\@journalshort{Biomechanics}
    \gdef\@doiabbr{biomechanics}
    \gdef\@ISSN{2673-7078}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{biomed}{%
    \gdef\@journal{biomed}
    \gdef\@journalfull{BioMed}
    \gdef\@journalshort{BioMed}
    \gdef\@doiabbr{biomed}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{biomedicines}{%
    \gdef\@journal{biomedicines}
    \gdef\@journalfull{Biomedicines}
    \gdef\@journalshort{Biomedicines}
    \gdef\@doiabbr{biomedicines}
    \gdef\@ISSN{2227-9059}
    \gdef\@societyowner{}
}
\DeclareOption{biomedinformatics}{%
    \gdef\@journal{biomedinformatics}
    \gdef\@journalfull{BioMedInformatics}
    \gdef\@journalshort{BioMedInformatics}
    \gdef\@doiabbr{biomedinformatics}
    \gdef\@ISSN{2673-7426}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{biomimetics}{%
    \gdef\@journal{biomimetics}
    \gdef\@journalfull{Biomimetics}
    \gdef\@journalshort{Biomimetics}
    \gdef\@doiabbr{biomimetics}
    \gdef\@ISSN{2313-7673}
    \gdef\@societyowner{}
}
\DeclareOption{biomolecules}{%
    \gdef\@journal{biomolecules}
    \gdef\@journalfull{Biomolecules}
    \gdef\@journalshort{Biomolecules}
    \gdef\@doiabbr{biom}
    \gdef\@ISSN{2218-273X}
    \gdef\@societyowner{}
}
\DeclareOption{biophysica}{%
    \gdef\@journal{biophysica}
    \gdef\@journalfull{Biophysica}
    \gdef\@journalshort{Biophysica}
    \gdef\@doiabbr{biophysica}
    \gdef\@ISSN{2673-4125}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{biosensors}{%
    \gdef\@journal{biosensors}
    \gdef\@journalfull{Biosensors}
    \gdef\@journalshort{Biosensors}
    \gdef\@doiabbr{bios}
    \gdef\@ISSN{2079-6374}
    \gdef\@societyowner{}
}
\DeclareOption{biotech}{%
    \gdef\@journal{biotech}
    \gdef\@journalfull{BioTech}
    \gdef\@journalshort{BioTech}
    \gdef\@doiabbr{biotech}
    \gdef\@ISSN{2673-6284}
    \gdef\@societyowner{}
}
\DeclareOption{birds}{%
    \gdef\@journal{birds}
    \gdef\@journalfull{Birds}
    \gdef\@journalshort{Birds}
    \gdef\@doiabbr{birds}
    \gdef\@ISSN{2673-6004}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{blockchains}{%
    \gdef\@journal{blockchains}
    \gdef\@journalfull{Blockchains}
    \gdef\@journalshort{Blockchains}
    \gdef\@doiabbr{blockchains}
    \gdef\@ISSN{2813-5288}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{bloods}{%
    \gdef\@journal{bloods}
    \gdef\@journalfull{Bloods}
    \gdef\@journalshort{Bloods}
    \gdef\@doiabbr{bloods}
    \gdef\@ISSN{2673-415X}
    \gdef\@societyowner{}
}
\DeclareOption{blsf}{%
    \gdef\@journal{blsf}
    \gdef\@journalfull{Biology and Life Sciences Forum}
    \gdef\@journalshort{Biol. Life Sci. Forum}
    \gdef\@doiabbr{blsf}
    \gdef\@ISSN{2673-9976}
    \gdef\@societyowner{}
}
\DeclareOption{brainsci}{%
    \gdef\@journal{brainsci}
    \gdef\@journalfull{Brain Sciences}
    \gdef\@journalshort{Brain Sci.}
    \gdef\@doiabbr{brainsci}
    \gdef\@ISSN{2076-3425}
    \gdef\@societyowner{}
}
\DeclareOption{breath}{%
    \gdef\@journal{breath}
    \gdef\@journalfull{Breath}
    \gdef\@journalshort{Breath}
    \gdef\@doiabbr{breath}
    \gdef\@ISSN{}
    \gdef\@societyowner{}
}
\DeclareOption{buildings}{%
    \gdef\@journal{buildings}
    \gdef\@journalfull{Buildings}
    \gdef\@journalshort{Buildings}
    \gdef\@doiabbr{buildings}
    \gdef\@ISSN{2075-5309}
    \gdef\@societyowner{}
}
\DeclareOption{businesses}{%
    \gdef\@journal{businesses}
    \gdef\@journalfull{Businesses}
    \gdef\@journalshort{Businesses}
    \gdef\@doiabbr{businesses}
    \gdef\@ISSN{2673-7116}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{cancers}{%
    \gdef\@journal{cancers}
    \gdef\@journalfull{Cancers}
    \gdef\@journalshort{Cancers}
    \gdef\@doiabbr{cancers}
    \gdef\@ISSN{2072-6694}
    \gdef\@societyowner{}
}
\DeclareOption{carbon}{%
    \gdef\@journal{carbon}
    \gdef\@journalfull{C}
    \gdef\@journalshort{C}
    \gdef\@doiabbr{c}
    \gdef\@ISSN{2311-5629}
    \gdef\@societyowner{}
}
\DeclareOption{cardiogenetics}{%
    \gdef\@journal{cardiogenetics}
    \gdef\@journalfull{Cardiogenetics}
    \gdef\@journalshort{Cardiogenetics}
    \gdef\@doiabbr{cardiogenetics}
    \gdef\@ISSN{2035-8148}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{catalysts}{%
    \gdef\@journal{catalysts}
    \gdef\@journalfull{Catalysts}
    \gdef\@journalshort{Catalysts}
    \gdef\@doiabbr{catal}
    \gdef\@ISSN{2073-4344}
    \gdef\@societyowner{}
}
\DeclareOption{cells}{%
    \gdef\@journal{cells}
    \gdef\@journalfull{Cells}
    \gdef\@journalshort{Cells}
    \gdef\@doiabbr{cells}
    \gdef\@ISSN{2073-4409}
    \gdef\@societyowner{}
}
\DeclareOption{ceramics}{%
    \gdef\@journal{ceramics}
    \gdef\@journalfull{Ceramics}
    \gdef\@journalshort{Ceramics}
    \gdef\@doiabbr{ceramics}
    \gdef\@ISSN{2571-6131}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{challenges}{%
    \gdef\@journal{challenges}
    \gdef\@journalfull{Challenges}
    \gdef\@journalshort{Challenges}
    \gdef\@doiabbr{challe}
    \gdef\@ISSN{2078-1547}
    \gdef\@societyowner{}
}
\DeclareOption{chemengineering}{%
    \gdef\@journal{chemengineering}
    \gdef\@journalfull{ChemEngineering}
    \gdef\@journalshort{ChemEngineering}
    \gdef\@doiabbr{chemengineering}
    \gdef\@ISSN{2305-7084}
    \gdef\@societyowner{}
}
\DeclareOption{chemistry}{%
    \gdef\@journal{chemistry}
    \gdef\@journalfull{Chemistry}
    \gdef\@journalshort{Chemistry}
    \gdef\@doiabbr{chemistry}
    \gdef\@ISSN{2624-8549}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{chemosensors}{%
    \gdef\@journal{chemosensors}
    \gdef\@journalfull{Chemosensors}
    \gdef\@journalshort{Chemosensors}
    \gdef\@doiabbr{chemosensors}
    \gdef\@ISSN{2227-9040}
    \gdef\@societyowner{}
}
\DeclareOption{chemproc}{%
    \gdef\@journal{chemproc}
    \gdef\@journalfull{Chemistry Proceedings}
    \gdef\@journalshort{Chem. Proc.}
    \gdef\@doiabbr{chemproc}
    \gdef\@ISSN{2673-4583}
    \gdef\@societyowner{}
}
\DeclareOption{children}{%
    \gdef\@journal{children}
    \gdef\@journalfull{Children}
    \gdef\@journalshort{Children}
    \gdef\@doiabbr{children}
    \gdef\@ISSN{2227-9067}
    \gdef\@societyowner{}
}
\DeclareOption{chips}{%
    \gdef\@journal{chips}
    \gdef\@journalfull{Chips}
    \gdef\@journalshort{Chips}
    \gdef\@doiabbr{chips}
    \gdef\@ISSN{2674-0729}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{cimb}{%
    \gdef\@journal{cimb}
    \gdef\@journalfull{Current Issues in Molecular Biology}
    \gdef\@journalshort{Curr. Issues Mol. Biol.}
    \gdef\@doiabbr{cimb}
    \gdef\@ISSN{1467-3045}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{civileng}{%
    \gdef\@journal{civileng}
    \gdef\@journalfull{CivilEng}
    \gdef\@journalshort{CivilEng}
    \gdef\@doiabbr{civileng}
    \gdef\@ISSN{2673-4109}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{cleantechnol}{%
    \gdef\@journal{cleantechnol}
    \gdef\@journalfull{Clean Technologies}
    \gdef\@journalshort{Clean Technol.}
    \gdef\@doiabbr{cleantechnol}
    \gdef\@ISSN{2571-8797}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{climate}{%
    \gdef\@journal{climate}
    \gdef\@journalfull{Climate}
    \gdef\@journalshort{Climate}
    \gdef\@doiabbr{cli}
    \gdef\@ISSN{2225-1154}
    \gdef\@societyowner{}
}
\DeclareOption{clinpract}{%
    \gdef\@journal{clinpract}
    \gdef\@journalfull{Clinics and Practice}
    \gdef\@journalshort{Clin. Pract.}
    \gdef\@doiabbr{clinpract}
    \gdef\@ISSN{2039-7283}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{clockssleep}{%
    \gdef\@journal{clockssleep}
    \gdef\@journalfull{Clocks \& Sleep}
    \gdef\@journalshort{Clocks\&Sleep}
    \gdef\@doiabbr{clockssleep}
    \gdef\@ISSN{2624-5175}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{cmd}{%
    \gdef\@journal{cmd}
    \gdef\@journalfull{Corrosion and Materials Degradation}
    \gdef\@journalshort{Corros. Mater. Degrad.}
    \gdef\@doiabbr{cmd}
    \gdef\@ISSN{2624-5558}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{coasts}{%
    \gdef\@journal{coasts}
    \gdef\@journalfull{Coasts}
    \gdef\@journalshort{Coasts}
    \gdef\@doiabbr{coasts}
    \gdef\@ISSN{2673-964X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{coatings}{%
    \gdef\@journal{coatings}
    \gdef\@journalfull{Coatings}
    \gdef\@journalshort{Coatings}
    \gdef\@doiabbr{coatings}
    \gdef\@ISSN{2079-6412}
    \gdef\@societyowner{}
}
\DeclareOption{colloids}{%
    \gdef\@journal{colloids}
    \gdef\@journalfull{Colloids and Interfaces}
    \gdef\@journalshort{Colloids Interfaces}
    \gdef\@doiabbr{colloids}
    \gdef\@ISSN{2504-5377}
    \gdef\@societyowner{}
}
\DeclareOption{colorants}{%
    \gdef\@journal{colorants}
    \gdef\@journalfull{Colorants}
    \gdef\@journalshort{Colorants}
    \gdef\@doiabbr{colorants}
    \gdef\@ISSN{2079-6447}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{commodities}{%
    \gdef\@journal{commodities}
    \gdef\@journalfull{Commodities}
    \gdef\@journalshort{Commodities}
    \gdef\@doiabbr{commodities}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{complications}{%
    \gdef\@journal{complications}
    \gdef\@journalfull{Complications}
    \gdef\@journalshort{Complications}
    \gdef\@doiabbr{complications}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{compounds}{%
    \gdef\@journal{compounds}
    \gdef\@journalfull{Compounds}
    \gdef\@journalshort{Compounds}
    \gdef\@doiabbr{compounds}
    \gdef\@ISSN{2673-6918}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{computation}{%
    \gdef\@journal{computation}
    \gdef\@journalfull{Computation}
    \gdef\@journalshort{Computation}
    \gdef\@doiabbr{computation}
    \gdef\@ISSN{2079-3197}
    \gdef\@societyowner{}
}
\DeclareOption{computers}{%
    \gdef\@journal{computers}
    \gdef\@journalfull{Computers}
    \gdef\@journalshort{Computers}
    \gdef\@doiabbr{computers}
    \gdef\@ISSN{2073-431X}
    \gdef\@societyowner{}
}
\DeclareOption{condensedmatter}{%
    \gdef\@journal{condensedmatter}
    \gdef\@journalfull{Condensed Matter}
    \gdef\@journalshort{Condens. Matter}
    \gdef\@doiabbr{condmat}
    \gdef\@ISSN{2410-3896}
    \gdef\@societyowner{}
}
\DeclareOption{conservation}{%
    \gdef\@journal{conservation}
    \gdef\@journalfull{Conservation}
    \gdef\@journalshort{Conservation}
    \gdef\@doiabbr{conservation}
    \gdef\@ISSN{2673-7159}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{constrmater}{%
    \gdef\@journal{constrmater}
    \gdef\@journalfull{Construction Materials}
    \gdef\@journalshort{Constr. Mater.}
    \gdef\@doiabbr{constrmater}
    \gdef\@ISSN{2673-7108}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{cosmetics}{%
    \gdef\@journal{cosmetics}
    \gdef\@journalfull{Cosmetics}
    \gdef\@journalshort{Cosmetics}
    \gdef\@doiabbr{cosmetics}
    \gdef\@ISSN{2079-9284}
    \gdef\@societyowner{}
}
\DeclareOption{covid}{%
    \gdef\@journal{covid}
    \gdef\@journalfull{COVID}
    \gdef\@journalshort{COVID}
    \gdef\@doiabbr{covid}
    \gdef\@ISSN{2673-8112}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{crops}{%
    \gdef\@journal{crops}
    \gdef\@journalfull{Crops}
    \gdef\@journalshort{Crops}
    \gdef\@doiabbr{crops}
    \gdef\@ISSN{2673-7655}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{cryo}{%
    \gdef\@journal{cryo}
    \gdef\@journalfull{Cryo}
    \gdef\@journalshort{Cryo}
    \gdef\@doiabbr{cryo}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{cryptography}{%
    \gdef\@journal{cryptography}
    \gdef\@journalfull{Cryptography}
    \gdef\@journalshort{Cryptography}
    \gdef\@doiabbr{cryptography}
    \gdef\@ISSN{2410-387X}
    \gdef\@societyowner{}
}
\DeclareOption{crystals}{%
    \gdef\@journal{crystals}
    \gdef\@journalfull{Crystals}
    \gdef\@journalshort{Crystals}
    \gdef\@doiabbr{cryst}
    \gdef\@ISSN{2073-4352}
    \gdef\@societyowner{}
}
\DeclareOption{csmf}{%
    \gdef\@journal{csmf}
    \gdef\@journalfull{Computer Sciences \& Mathematics Forum}
    \gdef\@journalshort{Comput. Sci. Math. Forum}
    \gdef\@doiabbr{csmf}
    \gdef\@ISSN{2813-0324}
    \gdef\@societyowner{}
}
\DeclareOption{ctn}{%
    \gdef\@journal{ctn}
    \gdef\@journalfull{Clinical and Translational Neuroscience}
    \gdef\@journalshort{Clin. Transl. Neurosci.}
    \gdef\@doiabbr{ctn}
    \gdef\@ISSN{2514-183X}
    \gdef\@societyowner{Swiss Federation of Clinical Neuro-Societies}
}
\DeclareOption{curroncol}{%
    \gdef\@journal{curroncol}
    \gdef\@journalfull{Current Oncology}
    \gdef\@journalshort{Curr. Oncol.}
    \gdef\@doiabbr{curroncol}
    \gdef\@ISSN{1718-7729}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{cyber}{%
    \gdef\@journal{cyber}
    \gdef\@journalfull{Cyber}
    \gdef\@journalshort{Cyber}
    \gdef\@doiabbr{cyber}
    \gdef\@ISSN{2624-800X}
    \gdef\@societyowner{}
}
\DeclareOption{dairy}{%
    \gdef\@journal{dairy}
    \gdef\@journalfull{Dairy}
    \gdef\@journalshort{Dairy}
    \gdef\@doiabbr{dairy}
    \gdef\@ISSN{2624-862X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{data}{%
    \gdef\@journal{data}
    \gdef\@journalfull{Data}
    \gdef\@journalshort{Data}
    \gdef\@doiabbr{data}
    \gdef\@ISSN{2306-5729}
    \gdef\@societyowner{}
}
\DeclareOption{ddc}{%
    \gdef\@journal{ddc}
    \gdef\@journalfull{Drugs and Drug Candidates}
    \gdef\@journalshort{Drugs Drug Candidates}
    \gdef\@doiabbr{ddc}
    \gdef\@ISSN{2813-2998}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{dentistry}{%
    \gdef\@journal{dentistry}
    \gdef\@journalfull{Dentistry Journal}
    \gdef\@journalshort{Dent. J.}
    \gdef\@doiabbr{dj}
    \gdef\@ISSN{2304-6767}
    \gdef\@societyowner{}
}
\DeclareOption{dermato}{%
    \gdef\@journal{dermato}
    \gdef\@journalfull{Dermato}
    \gdef\@journalshort{Dermato}
    \gdef\@doiabbr{dermato}
    \gdef\@ISSN{2673-6179}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{dermatopathology}{%
    \gdef\@journal{dermatopathology}
    \gdef\@journalfull{Dermatopathology}
    \gdef\@journalshort{Dermatopathology}
    \gdef\@doiabbr{dermatopathology}
    \gdef\@ISSN{2296-3529}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{European Society of Dermatopathology}
}
\DeclareOption{designs}{%
    \gdef\@journal{designs}
    \gdef\@journalfull{Designs}
    \gdef\@journalshort{Designs}
    \gdef\@doiabbr{designs}
    \gdef\@ISSN{2411-9660}
    \gdef\@societyowner{}
}
\DeclareOption{devices}{%
    \gdef\@journal{devices}
    \gdef\@journalfull{Devices}
    \gdef\@journalshort{Devices}
    \gdef\@doiabbr{devices}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{diabetology}{%
    \gdef\@journal{diabetology}
    \gdef\@journalfull{Diabetology}
    \gdef\@journalshort{Diabetology}
    \gdef\@doiabbr{diabetology}
    \gdef\@ISSN{2673-4540}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{diagnostics}{%
    \gdef\@journal{diagnostics}
    \gdef\@journalfull{Diagnostics}
    \gdef\@journalshort{Diagnostics}
    \gdef\@doiabbr{diagnostics}
    \gdef\@ISSN{2075-4418}
    \gdef\@societyowner{}
}
\DeclareOption{dietetics}{%
    \gdef\@journal{dietetics}
    \gdef\@journalfull{Dietetics}
    \gdef\@journalshort{Dietetics}
    \gdef\@doiabbr{dietetics}
    \gdef\@ISSN{2674-0311}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{digital}{%
    \gdef\@journal{digital}
    \gdef\@journalfull{Digital}
    \gdef\@journalshort{Digital}
    \gdef\@doiabbr{digital}
    \gdef\@ISSN{2673-6470}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{disabilities}{%
    \gdef\@journal{disabilities}
    \gdef\@journalfull{Disabilities}
    \gdef\@journalshort{Disabilities}
    \gdef\@doiabbr{disabilities}
    \gdef\@ISSN{2673-7272}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{diseases}{%
    \gdef\@journal{diseases}
    \gdef\@journalfull{Diseases}
    \gdef\@journalshort{Diseases}
    \gdef\@doiabbr{diseases}
    \gdef\@ISSN{2079-9721}
    \gdef\@societyowner{}
}
\DeclareOption{diversity}{%
    \gdef\@journal{diversity}
    \gdef\@journalfull{Diversity}
    \gdef\@journalshort{Diversity}
    \gdef\@doiabbr{d}
    \gdef\@ISSN{1424-2818}
    \gdef\@societyowner{}
}
\DeclareOption{dna}{%
    \gdef\@journal{dna}
    \gdef\@journalfull{DNA}
    \gdef\@journalshort{DNA}
    \gdef\@doiabbr{dna}
    \gdef\@ISSN{2673-8856}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{drones}{%
    \gdef\@journal{drones}
    \gdef\@journalfull{Drones}
    \gdef\@journalshort{Drones}
    \gdef\@doiabbr{drones}
    \gdef\@ISSN{2504-446X}
    \gdef\@societyowner{}
}
\DeclareOption{dynamics}{%
    \gdef\@journal{dynamics}
    \gdef\@journalfull{Dynamics}
    \gdef\@journalshort{Dynamics}
    \gdef\@doiabbr{dynamics}
    \gdef\@ISSN{2673-8716}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{earth}{%
    \gdef\@journal{earth}
    \gdef\@journalfull{Earth}
    \gdef\@journalshort{Earth}
    \gdef\@doiabbr{earth}
    \gdef\@ISSN{2673-4834}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{ebj}{%
    \gdef\@journal{ebj}
    \gdef\@journalfull{European Burn Journal}
    \gdef\@journalshort{Eur. Burn J.}
    \gdef\@doiabbr{ebj}
    \gdef\@ISSN{2673-1991}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{European Burns Association}
}
\DeclareOption{ecm}{%
    \gdef\@journal{ecm}
    \gdef\@journalfull{Emergency Care and Medicine}
    \gdef\@journalshort{Emerg. Care Med.}
    \gdef\@doiabbr{ecm}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{ecologies}{%
    \gdef\@journal{ecologies}
    \gdef\@journalfull{Ecologies}
    \gdef\@journalshort{Ecologies}
    \gdef\@doiabbr{ecologies}
    \gdef\@ISSN{2673-4133}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{econometrics}{%
    \gdef\@journal{econometrics}
    \gdef\@journalfull{Econometrics}
    \gdef\@journalshort{Econometrics}
    \gdef\@doiabbr{econometrics}
    \gdef\@ISSN{2225-1146}
    \gdef\@societyowner{}
}
\DeclareOption{economies}{%
    \gdef\@journal{economies}
    \gdef\@journalfull{Economies}
    \gdef\@journalshort{Economies}
    \gdef\@doiabbr{economies}
    \gdef\@ISSN{2227-7099}
    \gdef\@societyowner{}
}
\DeclareOption{education}{%
    \gdef\@journal{education}
    \gdef\@journalfull{Education Sciences}
    \gdef\@journalshort{Educ. Sci.}
    \gdef\@doiabbr{educsci}
    \gdef\@ISSN{2227-7102}
    \gdef\@societyowner{}
}
\DeclareOption{ejihpe}{%
    \gdef\@journal{ejihpe}
    \gdef\@journalfull{European Journal of Investigation in Health, Psychology and Education}
    \gdef\@journalshort{Eur. J. Investig. Health Psychol. Educ.}
    \gdef\@doiabbr{ejihpe}
    \gdef\@ISSN{2254-9625}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{University Association of Education and Psychology}
}
\DeclareOption{electricity}{%
    \gdef\@journal{electricity}
    \gdef\@journalfull{Electricity}
    \gdef\@journalshort{Electricity}
    \gdef\@doiabbr{electricity}
    \gdef\@ISSN{2673-4826}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{electrochem}{%
    \gdef\@journal{electrochem}
    \gdef\@journalfull{Electrochem}
    \gdef\@journalshort{Electrochem}
    \gdef\@doiabbr{electrochem}
    \gdef\@ISSN{2673-3293}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{electronicmat}{%
    \gdef\@journal{electronicmat}
    \gdef\@journalfull{Electronic Materials}
    \gdef\@journalshort{Electron. Mater.}
    \gdef\@doiabbr{electronicmat}
    \gdef\@ISSN{2673-3978}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{electronics}{%
    \gdef\@journal{electronics}
    \gdef\@journalfull{Electronics}
    \gdef\@journalshort{Electronics}
    \gdef\@doiabbr{electronics}
    \gdef\@ISSN{2079-9292}
    \gdef\@societyowner{}
}
\DeclareOption{encyclopedia}{%
    \gdef\@journal{encyclopedia}
    \gdef\@journalfull{Encyclopedia}
    \gdef\@journalshort{Encyclopedia}
    \gdef\@doiabbr{encyclopedia}
    \gdef\@ISSN{2673-8392}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{endocrines}{%
    \gdef\@journal{endocrines}
    \gdef\@journalfull{Endocrines}
    \gdef\@journalshort{Endocrines}
    \gdef\@doiabbr{endocrines}
    \gdef\@ISSN{2673-396X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{energies}{%
    \gdef\@journal{energies}
    \gdef\@journalfull{Energies}
    \gdef\@journalshort{Energies}
    \gdef\@doiabbr{en}
    \gdef\@ISSN{1996-1073}
    \gdef\@societyowner{}
}
\DeclareOption{eng}{%
    \gdef\@journal{eng}
    \gdef\@journalfull{Eng}
    \gdef\@journalshort{Eng}
    \gdef\@doiabbr{eng}
    \gdef\@ISSN{2673-4117}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{engproc}{%
    \gdef\@journal{engproc}
    \gdef\@journalfull{Engineering Proceedings}
    \gdef\@journalshort{Eng. Proc.}
    \gdef\@doiabbr{engproc}
    \gdef\@ISSN{2673-4591}
    \gdef\@societyowner{}
}
%\DeclareOption{ent}{%
%	\gdef\@journal{ent}
%	\gdef\@journalfull{}
%	\gdef\@journalshort{}
%	\gdef\@doiabbr{}
%	\gdef\@ISSN{}
%	\gdef\@continuouspages{yes}
%	\gdef\@societyowner{}
%}
\DeclareOption{entomology}{%
    \gdef\@journal{entomology}
    \gdef\@journalfull{Entomology}
    \gdef\@journalshort{Entomology}
    \gdef\@doiabbr{entomology}
    \gdef\@ISSN{2813-0502}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{entropy}{%
    \gdef\@journal{entropy}
    \gdef\@journalfull{Entropy}
    \gdef\@journalshort{Entropy}
    \gdef\@doiabbr{e}
    \gdef\@ISSN{1099-4300}
    \gdef\@societyowner{}
}
\DeclareOption{environments}{%
    \gdef\@journal{environments}
    \gdef\@journalfull{Environments}
    \gdef\@journalshort{Environments}
    \gdef\@doiabbr{environments}
    \gdef\@ISSN{2076-3298}
    \gdef\@societyowner{}
}
\DeclareOption{environsciproc}{%
    \gdef\@journal{environsciproc}
    \gdef\@journalfull{Environmental Sciences Proceedings}
    \gdef\@journalshort{Environ. Sci. Proc.}
    \gdef\@doiabbr{environsciproc}
    \gdef\@ISSN{2673-4931}
    \gdef\@societyowner{}
}
\DeclareOption{epidemiologia}{%
    \gdef\@journal{epidemiologia}
    \gdef\@journalfull{Epidemiologia}
    \gdef\@journalshort{Epidemiologia}
    \gdef\@doiabbr{epidemiologia}
    \gdef\@ISSN{2673-3986}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{epigenomes}{%
    \gdef\@journal{epigenomes}
    \gdef\@journalfull{Epigenomes}
    \gdef\@journalshort{Epigenomes}
    \gdef\@doiabbr{epigenomes}
    \gdef\@ISSN{2075-4655}
    \gdef\@societyowner{}
}
\DeclareOption{esa}{%
    \gdef\@journal{esa}
    \gdef\@journalfull{Energy Storage and Applications}
    \gdef\@journalshort{Energy Storage Appl.}
    \gdef\@doiabbr{esa}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{est}{%
    \gdef\@journal{est}
    \gdef\@journalfull{Electrochemical Science and Technology}
    \gdef\@journalshort{Electrochem. Sci. Technol.}
    \gdef\@doiabbr{}
    \gdef\@ISSN{}
    \gdef\@societyowner{}
}
\DeclareOption{fermentation}{%
    \gdef\@journal{fermentation}
    \gdef\@journalfull{Fermentation}
    \gdef\@journalshort{Fermentation}
    \gdef\@doiabbr{fermentation}
    \gdef\@ISSN{2311-5637}
    \gdef\@societyowner{}
}
\DeclareOption{fibers}{%
    \gdef\@journal{fibers}
    \gdef\@journalfull{Fibers}
    \gdef\@journalshort{Fibers}
    \gdef\@doiabbr{fib}
    \gdef\@ISSN{2079-6439}
    \gdef\@societyowner{}
}
\DeclareOption{fintech}{%
    \gdef\@journal{fintech}
    \gdef\@journalfull{FinTech}
    \gdef\@journalshort{FinTech}
    \gdef\@doiabbr{fintech}
    \gdef\@ISSN{2674-1032}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{fire}{%
    \gdef\@journal{fire}
    \gdef\@journalfull{Fire}
    \gdef\@journalshort{Fire}
    \gdef\@doiabbr{fire}
    \gdef\@ISSN{2571-6255}
    \gdef\@societyowner{}
}
\DeclareOption{fishes}{%
    \gdef\@journal{fishes}
    \gdef\@journalfull{Fishes}
    \gdef\@journalshort{Fishes}
    \gdef\@doiabbr{fishes}
    \gdef\@ISSN{2410-3888}
    \gdef\@societyowner{}
}
\DeclareOption{fluids}{%
    \gdef\@journal{fluids}
    \gdef\@journalfull{Fluids}
    \gdef\@journalshort{Fluids}
    \gdef\@doiabbr{fluids}
    \gdef\@ISSN{2311-5521}
    \gdef\@societyowner{}
}
\DeclareOption{foods}{%
    \gdef\@journal{foods}
    \gdef\@journalfull{Foods}
    \gdef\@journalshort{Foods}
    \gdef\@doiabbr{foods}
    \gdef\@ISSN{2304-8158}
    \gdef\@societyowner{}
}
\DeclareOption{forecasting}{%
    \gdef\@journal{forecasting}
    \gdef\@journalfull{Forecasting}
    \gdef\@journalshort{Forecasting}
    \gdef\@doiabbr{forecast}
    \gdef\@ISSN{2571-9394}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{forensicsci}{%
    \gdef\@journal{forensicsci}
    \gdef\@journalfull{Forensic Sciences}
    \gdef\@journalshort{Forensic Sci.}
    \gdef\@doiabbr{forensicsci}
    \gdef\@ISSN{2673-6756}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{forests}{%
    \gdef\@journal{forests}
    \gdef\@journalfull{Forests}
    \gdef\@journalshort{Forests}
    \gdef\@doiabbr{f}
    \gdef\@ISSN{1999-4907}
    \gdef\@societyowner{}
}
\DeclareOption{fossstud}{%
    \gdef\@journal{fossstud}
    \gdef\@journalfull{Fossil Studies}
    \gdef\@journalshort{Foss. Stud.}
    \gdef\@doiabbr{fossils}
    \gdef\@ISSN{2813-6284}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{foundations}{%
    \gdef\@journal{foundations}
    \gdef\@journalfull{Foundations}
    \gdef\@journalshort{Foundations}
    \gdef\@doiabbr{foundations}
    \gdef\@ISSN{2673-9321}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{fractalfract}{%
    \gdef\@journal{fractalfract}
    \gdef\@journalfull{Fractal and Fractional}
    \gdef\@journalshort{Fractal Fract.}
    \gdef\@doiabbr{fractalfract}
    \gdef\@ISSN{2504-3110}
    \gdef\@societyowner{}
}
\DeclareOption{fuels}{%
    \gdef\@journal{fuels}
    \gdef\@journalfull{Fuels}
    \gdef\@journalshort{Fuels}
    \gdef\@doiabbr{fuels}
    \gdef\@ISSN{2673-3994}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{future}{%
    \gdef\@journal{future}
    \gdef\@journalfull{Future}
    \gdef\@journalshort{Future}
    \gdef\@doiabbr{future}
    \gdef\@ISSN{2813-2882}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{futureinternet}{%
    \gdef\@journal{futureinternet}
    \gdef\@journalfull{Future Internet}
    \gdef\@journalshort{Future Internet}
    \gdef\@doiabbr{fi}
    \gdef\@ISSN{1999-5903}
    \gdef\@societyowner{}
}
%\DeclareOption{futureparasites}{%
%	\gdef\@journal{futureparasites}
%	\gdef\@journalfull{}
%	\gdef\@journalshort{}
%	\gdef\@doiabbr{}
%	\gdef\@ISSN{}
%	\gdef\@continuouspages{yes}
%	\gdef\@societyowner{}
%}
\DeclareOption{futurepharmacol}{%
    \gdef\@journal{futurepharmacol}
    \gdef\@journalfull{Future Pharmacology}
    \gdef\@journalshort{Future Pharmacol.}
    \gdef\@doiabbr{futurepharmacol}
    \gdef\@ISSN{2673-9879}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{futurephys}{%
    \gdef\@journal{futurephys}
    \gdef\@journalfull{Future Physics}
    \gdef\@journalshort{Future Phys.}
    \gdef\@doiabbr{futurephys}
    \gdef\@ISSN{2624-6503}
    \gdef\@societyowner{}
}
\DeclareOption{futuretransp}{%
    \gdef\@journal{futuretransp}
    \gdef\@journalfull{Future Transportation}
    \gdef\@journalshort{Future Transp.}
    \gdef\@doiabbr{futuretransp}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{galaxies}{%
    \gdef\@journal{galaxies}
    \gdef\@journalfull{Galaxies}
    \gdef\@journalshort{Galaxies}
    \gdef\@doiabbr{galaxies}
    \gdef\@ISSN{2075-4434}
    \gdef\@societyowner{}
}
\DeclareOption{games}{%
    \gdef\@journal{games}
    \gdef\@journalfull{Games}
    \gdef\@journalshort{Games}
    \gdef\@doiabbr{g}
    \gdef\@ISSN{2073-4336}
    \gdef\@societyowner{}
}
\DeclareOption{gases}{%
    \gdef\@journal{gases}
    \gdef\@journalfull{Gases}
    \gdef\@journalshort{Gases}
    \gdef\@doiabbr{gases}
    \gdef\@ISSN{2673-5628}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{gastroent}{%
    \gdef\@journal{gastroent}
    \gdef\@journalfull{Gastroenterology Insights}
    \gdef\@journalshort{Gastroenterol. Insights}
    \gdef\@doiabbr{gastroent}
    \gdef\@ISSN{2036-7422}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{gastrointestdisord}{%
    \gdef\@journal{gastrointestdisord}
    \gdef\@journalfull{Gastrointestinal Disorders}
    \gdef\@journalshort{Gastrointest. Disord.}
    \gdef\@doiabbr{gidisord}
    \gdef\@ISSN{2624-5647}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{gastronomy}{%
    \gdef\@journal{gastronomy}
    \gdef\@journalfull{Gastronomy}
    \gdef\@journalshort{Gastronomy}
    \gdef\@doiabbr{gastronomy}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{gels}{%
    \gdef\@journal{gels}
    \gdef\@journalfull{Gels}
    \gdef\@journalshort{Gels}
    \gdef\@doiabbr{gels}
    \gdef\@ISSN{2310-2861}
    \gdef\@societyowner{}
}
\DeclareOption{genealogy}{%
    \gdef\@journal{genealogy}
    \gdef\@journalfull{Genealogy}
    \gdef\@journalshort{Genealogy}
    \gdef\@doiabbr{genealogy}
    \gdef\@ISSN{2313-5778}
    \gdef\@societyowner{}
}
\DeclareOption{genes}{%
    \gdef\@journal{genes}
    \gdef\@journalfull{Genes}
    \gdef\@journalshort{Genes}
    \gdef\@doiabbr{genes}
    \gdef\@ISSN{2073-4425}
    \gdef\@societyowner{}
}
\DeclareOption{geographies}{%
    \gdef\@journal{geographies}
    \gdef\@journalfull{Geographies}
    \gdef\@journalshort{Geographies}
    \gdef\@doiabbr{geographies}
    \gdef\@ISSN{2673-7086}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{geohazards}{%
    \gdef\@journal{geohazards}
    \gdef\@journalfull{GeoHazards}
    \gdef\@journalshort{GeoHazards}
    \gdef\@doiabbr{geohazards}
    \gdef\@ISSN{2624-795X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{geomatics}{%
    \gdef\@journal{geomatics}
    \gdef\@journalfull{Geomatics}
    \gdef\@journalshort{Geomatics}
    \gdef\@doiabbr{geomatics}
    \gdef\@ISSN{2673-7418}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{geometry}{%
    \gdef\@journal{geometry}
    \gdef\@journalfull{Geometry}
    \gdef\@journalshort{Geometry}
    \gdef\@doiabbr{geometry}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{geosciences}{%
    \gdef\@journal{geosciences}
    \gdef\@journalfull{Geosciences}
    \gdef\@journalshort{Geosciences}
    \gdef\@doiabbr{geosciences}
    \gdef\@ISSN{2076-3263}
    \gdef\@societyowner{}
}
\DeclareOption{geotechnics}{%
    \gdef\@journal{geotechnics}
    \gdef\@journalfull{Geotechnics}
    \gdef\@journalshort{Geotechnics}
    \gdef\@doiabbr{geotechnics}
    \gdef\@ISSN{2673-7094}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{geriatrics}{%
    \gdef\@journal{geriatrics}
    \gdef\@journalfull{Geriatrics}
    \gdef\@journalshort{Geriatrics}
    \gdef\@doiabbr{geriatrics}
    \gdef\@ISSN{2308-3417}
    \gdef\@societyowner{}
}
\DeclareOption{glacies}{%
    \gdef\@journal{glacies}
    \gdef\@journalfull{Glacies}
    \gdef\@journalshort{Glacies}
    \gdef\@doiabbr{glacies}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{grasses}{%
    \gdef\@journal{grasses}
    \gdef\@journalfull{Grasses}
    \gdef\@journalshort{Grasses}
    \gdef\@doiabbr{grasses}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{gucdd}{%
    \gdef\@journal{gucdd}
    \gdef\@journalfull{Gout, Urate, and Crystal Deposition Disease}
    \gdef\@journalshort{Gout Urate Cryst. Depos. Dis.}
    \gdef\@doiabbr{gucdd}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{Gout, Hyperuricemia and Crystal Associated Disease Network}
}
\DeclareOption{hardware}{%
    \gdef\@journal{hardware}
    \gdef\@journalfull{Hardware}
    \gdef\@journalshort{Hardware}
    \gdef\@doiabbr{hardware}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{hazardousmatters}{%
    \gdef\@journal{hazardousmatters}
    \gdef\@journalfull{Hazardous Matters}
    \gdef\@journalshort{Hazard. Matters}
    \gdef\@doiabbr{}
    \gdef\@ISSN{0014-0014}
    \gdef\@societyowner{}
}
\DeclareOption{healthcare}{%
    \gdef\@journal{healthcare}
    \gdef\@journalfull{Healthcare}
    \gdef\@journalshort{Healthcare}
    \gdef\@doiabbr{healthcare}
    \gdef\@ISSN{2227-9032}
    \gdef\@societyowner{}
}
\DeclareOption{hearts}{%
    \gdef\@journal{hearts}
    \gdef\@journalfull{Hearts}
    \gdef\@journalshort{Hearts}
    \gdef\@doiabbr{hearts}
    \gdef\@ISSN{2673-3846}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{hemato}{%
    \gdef\@journal{hemato}
    \gdef\@journalfull{Hemato}
    \gdef\@journalshort{Hemato}
    \gdef\@doiabbr{hemato}
    \gdef\@ISSN{2673-6357}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{hematolrep}{%
    \gdef\@journal{hematolrep}
    \gdef\@journalfull{Hematology Reports}
    \gdef\@journalshort{Hematol. Rep.}
    \gdef\@doiabbr{hematolrep}
    \gdef\@ISSN{2038-8330}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{heritage}{%
    \gdef\@journal{heritage}
    \gdef\@journalfull{Heritage}
    \gdef\@journalshort{Heritage}
    \gdef\@doiabbr{heritage}
    \gdef\@ISSN{2571-9408}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{higheredu}{%
    \gdef\@journal{higheredu}
    \gdef\@journalfull{Trends in Higher Education}
    \gdef\@journalshort{Trends High. Educ.}
    \gdef\@doiabbr{higheredu}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{highthroughput}{%
    \gdef\@journal{highthroughput}
    \gdef\@journalfull{High-Throughput}
    \gdef\@journalshort{High-Throughput}
    \gdef\@doiabbr{ht}
    \gdef\@ISSN{2571-5135}
    \gdef\@societyowner{}
}
\DeclareOption{histories}{%
    \gdef\@journal{histories}
    \gdef\@journalfull{Histories}
    \gdef\@journalshort{Histories}
    \gdef\@doiabbr{histories}
    \gdef\@ISSN{2409-9252}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{horticulturae}{%
    \gdef\@journal{horticulturae}
    \gdef\@journalfull{Horticulturae}
    \gdef\@journalshort{Horticulturae}
    \gdef\@doiabbr{horticulturae}
    \gdef\@ISSN{2311-7524}
    \gdef\@societyowner{}
}
\DeclareOption{hospitals}{%
    \gdef\@journal{hospitals}
    \gdef\@journalfull{Hospitals}
    \gdef\@journalshort{Hospitals}
    \gdef\@doiabbr{hospitals}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{humanities}{%
    \gdef\@journal{humanities}
    \gdef\@journalfull{Humanities}
    \gdef\@journalshort{Humanities}
    \gdef\@doiabbr{h}
    \gdef\@ISSN{2076-0787}
    \gdef\@societyowner{}
}
\DeclareOption{humans}{%
    \gdef\@journal{humans}
    \gdef\@journalfull{Humans}
    \gdef\@journalshort{Humans}
    \gdef\@doiabbr{humans}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{hydrobiology}{%
    \gdef\@journal{hydrobiology}
    \gdef\@journalfull{Hydrobiology}
    \gdef\@journalshort{Hydrobiology}
    \gdef\@doiabbr{hydrobiology}
    \gdef\@ISSN{2673-9917}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{hydrogen}{%
    \gdef\@journal{hydrogen}
    \gdef\@journalfull{Hydrogen}
    \gdef\@journalshort{Hydrogen}
    \gdef\@doiabbr{hydrogen}
    \gdef\@ISSN{2673-4141}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{hydrology}{%
    \gdef\@journal{hydrology}
    \gdef\@journalfull{Hydrology}
    \gdef\@journalshort{Hydrology}
    \gdef\@doiabbr{hydrology}
    \gdef\@ISSN{2306-5338}
    \gdef\@societyowner{}
}
\DeclareOption{hygiene}{%
    \gdef\@journal{hygiene}
    \gdef\@journalfull{Hygiene}
    \gdef\@journalshort{Hygiene}
    \gdef\@doiabbr{hygiene}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{idr}{%
    \gdef\@journal{idr}
    \gdef\@journalfull{Infectious Disease Reports}
    \gdef\@journalshort{Infect. Dis. Rep.}
    \gdef\@doiabbr{idr}
    \gdef\@ISSN{2036-7449}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{iic}{%
    \gdef\@journal{iic}
    \gdef\@journalfull{Intelligent Infrastructure and Construction}
    \gdef\@journalshort{Intell. Infrastruct. Constr.}
    \gdef\@doiabbr{iic}
    \gdef\@ISSN{3042-4720}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{ijerph}{%
    \gdef\@journal{ijerph}
    \gdef\@journalfull{International Journal of Environmental Research and Public Health}
    \gdef\@journalshort{Int. J. Environ. Res. Public Health}
    \gdef\@doiabbr{ijerph}
    \gdef\@ISSN{1660-4601}
    \gdef\@societyowner{}
}
\DeclareOption{ijfs}{%
    \gdef\@journal{ijfs}
    \gdef\@journalfull{International Journal of Financial Studies}
    \gdef\@journalshort{Int. J. Financial Stud.}
    \gdef\@doiabbr{ijfs}
    \gdef\@ISSN{2227-7072}
    \gdef\@societyowner{}
}
\DeclareOption{ijgi}{%
    \gdef\@journal{ijgi}
    \gdef\@journalfull{ISPRS International Journal of Geo-Information}
    \gdef\@journalshort{ISPRS Int. J. Geo-Inf.}
    \gdef\@doiabbr{ijgi}
    \gdef\@ISSN{2220-9964}
    \gdef\@societyowner{International Society for Photogrammetry and Remote Sensing}
}
\DeclareOption{ijmd}{%
    \gdef\@journal{ijmd}
    \gdef\@journalfull{International Journal of Medical Devices}
    \gdef\@journalshort{Int. J. Med. Devices}
    \gdef\@doiabbr{ijmd}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{ijms}{%
    \gdef\@journal{ijms}
    \gdef\@journalfull{International Journal of Molecular Sciences}
    \gdef\@journalshort{Int. J. Mol. Sci.}
    \gdef\@doiabbr{ijms}
    \gdef\@ISSN{1422-0067}
    \gdef\@societyowner{}
}
\DeclareOption{ijns}{%
    \gdef\@journal{ijns}
    \gdef\@journalfull{International Journal of Neonatal Screening}
    \gdef\@journalshort{Int. J. Neonatal Screen.}
    \gdef\@doiabbr{ijns}
    \gdef\@ISSN{2409-515X}
    \gdef\@societyowner{International Society for Neonatal Screening}
}
\DeclareOption{ijpb}{%
    \gdef\@journal{ijpb}
    \gdef\@journalfull{International Journal of Plant Biology}
    \gdef\@journalshort{Int. J. Plant Biol.}
    \gdef\@doiabbr{ijpb}
    \gdef\@ISSN{2037-0164}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{ijt}{%
    \gdef\@journal{ijt}
    \gdef\@journalfull{International Journal of Topology}
    \gdef\@journalshort{Int. J. Topol.}
    \gdef\@doiabbr{ijt}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{ijtm}{%
    \gdef\@journal{ijtm}
    \gdef\@journalfull{International Journal of Translational Medicine}
    \gdef\@journalshort{Int. J. Transl. Med.}
    \gdef\@doiabbr{ijtm}
    \gdef\@ISSN{2673-8937}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{ijtpp}{%
    \gdef\@journal{ijtpp}
    \gdef\@journalfull{International Journal of Turbomachinery, Propulsion and Power}
    \gdef\@journalshort{Int. J. Turbomach. Propuls. Power}
    \gdef\@doiabbr{ijtpp}
    \gdef\@ISSN{2504-186X}
    \gdef\@societyowner{EUROTURBO European turbomachinery society}
}
\DeclareOption{ime}{%
    \gdef\@journal{ime}
    \gdef\@journalfull{International Medical Education}
    \gdef\@journalshort{Int. Med. Educ.}
    \gdef\@doiabbr{ime}
    \gdef\@ISSN{2813-141X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{Academic Society for International Medical Education}
}
\DeclareOption{immuno}{%
    \gdef\@journal{immuno}
    \gdef\@journalfull{Immuno}
    \gdef\@journalshort{Immuno}
    \gdef\@doiabbr{immuno}
    \gdef\@ISSN{2673-5601}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{informatics}{%
    \gdef\@journal{informatics}
    \gdef\@journalfull{Informatics}
    \gdef\@journalshort{Informatics}
    \gdef\@doiabbr{informatics}
    \gdef\@ISSN{2227-9709}
    \gdef\@societyowner{}
}
\DeclareOption{information}{%
    \gdef\@journal{information}
    \gdef\@journalfull{Information}
    \gdef\@journalshort{Information}
    \gdef\@doiabbr{info}
    \gdef\@ISSN{2078-2489}
    \gdef\@societyowner{}
}
\DeclareOption{infrastructures}{%
    \gdef\@journal{infrastructures}
    \gdef\@journalfull{Infrastructures}
    \gdef\@journalshort{Infrastructures}
    \gdef\@doiabbr{infrastructures}
    \gdef\@ISSN{2412-3811}
    \gdef\@societyowner{}
}
\DeclareOption{inorganics}{%
    \gdef\@journal{inorganics}
    \gdef\@journalfull{Inorganics}
    \gdef\@journalshort{Inorganics}
    \gdef\@doiabbr{inorganics}
    \gdef\@ISSN{2304-6740}
    \gdef\@societyowner{}
}
\DeclareOption{insects}{%
    \gdef\@journal{insects}
    \gdef\@journalfull{Insects}
    \gdef\@journalshort{Insects}
    \gdef\@doiabbr{insects}
    \gdef\@ISSN{2075-4450}
    \gdef\@societyowner{}
}
\DeclareOption{instruments}{%
    \gdef\@journal{instruments}
    \gdef\@journalfull{Instruments}
    \gdef\@journalshort{Instruments}
    \gdef\@doiabbr{instruments}
    \gdef\@ISSN{2410-390X}
    \gdef\@societyowner{}
}
\DeclareOption{inventions}{%
    \gdef\@journal{inventions}
    \gdef\@journalfull{Inventions}
    \gdef\@journalshort{Inventions}
    \gdef\@doiabbr{inventions}
    \gdef\@ISSN{2411-5134}
    \gdef\@societyowner{}
}
\DeclareOption{iot}{%
    \gdef\@journal{iot}
    \gdef\@journalfull{IoT}
    \gdef\@journalshort{IoT}
    \gdef\@doiabbr{iot}
    \gdef\@ISSN{2624-831X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{j}{%
    \gdef\@journal{j}
    \gdef\@journalfull{J}
    \gdef\@journalshort{J}
    \gdef\@doiabbr{j}
    \gdef\@ISSN{2571-8800}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jal}{%
    \gdef\@journal{jal}
    \gdef\@journalfull{Journal of Ageing and Longevity}
    \gdef\@journalshort{J. Ageing Longev.}
    \gdef\@doiabbr{jal}
    \gdef\@ISSN{2673-9259}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jcdd}{%
    \gdef\@journal{jcdd}
    \gdef\@journalfull{Journal of Cardiovascular Development and Disease}
    \gdef\@journalshort{J. Cardiovasc. Dev. Dis.}
    \gdef\@doiabbr{jcdd}
    \gdef\@ISSN{2308-3425}
    \gdef\@societyowner{}
}
\DeclareOption{jcm}{%
    \gdef\@journal{jcm}
    \gdef\@journalfull{Journal of Clinical Medicine}
    \gdef\@journalshort{J. Clin. Med.}
    \gdef\@doiabbr{jcm}
    \gdef\@ISSN{2077-0383}
    \gdef\@societyowner{}
}
\DeclareOption{jcp}{%
    \gdef\@journal{jcp}
    \gdef\@journalfull{Journal of Cybersecurity and Privacy}
    \gdef\@journalshort{J. Cybersecur. Priv.}
    \gdef\@doiabbr{jcp}
    \gdef\@ISSN{2624-800X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jcs}{%
    \gdef\@journal{jcs}
    \gdef\@journalfull{Journal of Composites Science}
    \gdef\@journalshort{J. Compos. Sci.}
    \gdef\@doiabbr{jcs}
    \gdef\@ISSN{2504-477X}
    \gdef\@societyowner{}
}
\DeclareOption{jcto}{%
    \gdef\@journal{jcto}
    \gdef\@journalfull{Journal of Clinical \& Translational Ophthalmology}
    \gdef\@journalshort{J. Clin. Transl. Ophthalmol.}
    \gdef\@doiabbr{jcto}
    \gdef\@ISSN{2813-1053}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jdad}{%
    \gdef\@journal{jdad}
    \gdef\@journalfull{Journal of Dementia and Alzheimer’s Disease}
    \gdef\@journalshort{J. Dement. Alzheimer's Dis.}
    \gdef\@doiabbr{jdad}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jdb}{%
    \gdef\@journal{jdb}
    \gdef\@journalfull{Journal of Developmental Biology}
    \gdef\@journalshort{J. Dev. Biol.}
    \gdef\@doiabbr{jdb}
    \gdef\@ISSN{2221-3759}
    \gdef\@societyowner{}
}
\DeclareOption{jeta}{%
    \gdef\@journal{jeta}
    \gdef\@journalfull{Journal of Experimental and Theoretical Analyses}
    \gdef\@journalshort{J. Exp. Theor. Anal.}
    \gdef\@doiabbr{jeta}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jfb}{%
    \gdef\@journal{jfb}
    \gdef\@journalfull{Journal of Functional Biomaterials}
    \gdef\@journalshort{J. Funct. Biomater.}
    \gdef\@doiabbr{jfb}
    \gdef\@ISSN{2079-4983}
    \gdef\@societyowner{}
}
\DeclareOption{jfmk}{%
    \gdef\@journal{jfmk}
    \gdef\@journalfull{Journal of Functional Morphology and Kinesiology}
    \gdef\@journalshort{J. Funct. Morphol. Kinesiol.}
    \gdef\@doiabbr{jfmk}
    \gdef\@ISSN{2411-5142}
    \gdef\@societyowner{}
}
\DeclareOption{jimaging}{%
    \gdef\@journal{jimaging}
    \gdef\@journalfull{Journal of Imaging}
    \gdef\@journalshort{J. Imaging}
    \gdef\@doiabbr{jimaging}
    \gdef\@ISSN{2313-433X}
    \gdef\@societyowner{}
}
\DeclareOption{jintelligence}{%
    \gdef\@journal{jintelligence}
    \gdef\@journalfull{Journal of Intelligence}
    \gdef\@journalshort{J. Intell.}
    \gdef\@doiabbr{jintelligence}
    \gdef\@ISSN{2079-3200}
    \gdef\@societyowner{}
}
\DeclareOption{jlpea}{%
    \gdef\@journal{jlpea}
    \gdef\@journalfull{Journal of Low Power Electronics and Applications}
    \gdef\@journalshort{J. Low Power Electron. Appl.}
    \gdef\@doiabbr{jlpea}
    \gdef\@ISSN{2079-9268}
    \gdef\@societyowner{}
}
\DeclareOption{jmahp}{%
    \gdef\@journal{jmahp}
    \gdef\@journalfull{Journal of Market Access \& Health Policy}
    \gdef\@journalshort{J. Mark. Access Health Policy}
    \gdef\@doiabbr{jmahp}
    \gdef\@ISSN{2001-6689}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{Market Access Society}
}
\DeclareOption{jmmp}{%
    \gdef\@journal{jmmp}
    \gdef\@journalfull{Journal of Manufacturing and Materials Processing}
    \gdef\@journalshort{J. Manuf. Mater. Process.}
    \gdef\@doiabbr{jmmp}
    \gdef\@ISSN{2504-4494}
    \gdef\@societyowner{}
}
\DeclareOption{jmp}{%
    \gdef\@journal{jmp}
    \gdef\@journalfull{Journal of Molecular Pathology}
    \gdef\@journalshort{J. Mol. Pathol.}
    \gdef\@doiabbr{jmp}
    \gdef\@ISSN{2673-5261}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jmse}{%
    \gdef\@journal{jmse}
    \gdef\@journalfull{Journal of Marine Science and Engineering}
    \gdef\@journalshort{J. Mar. Sci. Eng.}
    \gdef\@doiabbr{jmse}
    \gdef\@ISSN{2077-1312}
    \gdef\@societyowner{}
}
\DeclareOption{jne}{%
    \gdef\@journal{jne}
    \gdef\@journalfull{Journal of Nuclear Engineering}
    \gdef\@journalshort{J. Nucl. Eng.}
    \gdef\@doiabbr{jne}
    \gdef\@ISSN{2673-4362}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jnt}{%
    \gdef\@journal{jnt}
    \gdef\@journalfull{Journal of Nanotheranostics}
    \gdef\@journalshort{J. Nanotheranostics}
    \gdef\@doiabbr{jnt}
    \gdef\@ISSN{2624-845X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jof}{%
    \gdef\@journal{jof}
    \gdef\@journalfull{Journal of Fungi}
    \gdef\@journalshort{J. Fungi}
    \gdef\@doiabbr{jof}
    \gdef\@ISSN{2309-608X}
    \gdef\@societyowner{}
}
\DeclareOption{joitmc}{%
    \gdef\@journal{joitmc}
    \gdef\@journalfull{Journal of Open Innovation: Technology, Market, and Complexity}
    \gdef\@journalshort{J. Open Innov. Technol. Mark. Complex.}
    \gdef\@doiabbr{joitmc}
    \gdef\@ISSN{2199-8531}
    \gdef\@societyowner{}
}
\DeclareOption{joma}{%
    \gdef\@journal{joma}
    \gdef\@journalfull{Journal of the Oman Medical Association}
    \gdef\@journalshort{J. Oman Med. Assoc.}
    \gdef\@doiabbr{joma}
    \gdef\@ISSN{2813-8759}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{Oman Medical Association}
}
\DeclareOption{jor}{%
    \gdef\@journal{jor}
    \gdef\@journalfull{Journal of Respiration}
    \gdef\@journalshort{J. Respir.}
    \gdef\@doiabbr{jor}
    \gdef\@ISSN{2673-527X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{journalmedia}{%
    \gdef\@journal{journalmedia}
    \gdef\@journalfull{Journalism and Media}
    \gdef\@journalshort{Journal. Media}
    \gdef\@doiabbr{journalmedia}
    \gdef\@ISSN{2673-5172}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jox}{%
    \gdef\@journal{jox}
    \gdef\@journalfull{Journal of Xenobiotics}
    \gdef\@journalshort{J. Xenobiot.}
    \gdef\@doiabbr{jox}
    \gdef\@ISSN{2039-4713}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jpbi}{%
    \gdef\@journal{jpbi}
    \gdef\@journalfull{Journal of Pharmaceutical and BioTech Industry}
    \gdef\@journalshort{J. Pharm. BioTech Ind.}
    \gdef\@doiabbr{jpbi}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jpm}{%
    \gdef\@journal{jpm}
    \gdef\@journalfull{Journal of Personalized Medicine}
    \gdef\@journalshort{J. Pers. Med.}
    \gdef\@doiabbr{jpm}
    \gdef\@ISSN{2075-4426}
    \gdef\@societyowner{}
}
\DeclareOption{jrfm}{%
    \gdef\@journal{jrfm}
    \gdef\@journalfull{Journal of Risk and Financial Management}
    \gdef\@journalshort{J. Risk Financial Manag.}
    \gdef\@doiabbr{jrfm}
    \gdef\@ISSN{1911-8074}
    \gdef\@societyowner{}
}
\DeclareOption{jsan}{%
    \gdef\@journal{jsan}
    \gdef\@journalfull{Journal of Sensor and Actuator Networks}
    \gdef\@journalshort{J. Sens. Actuator Netw.}
    \gdef\@doiabbr{jsan}
    \gdef\@ISSN{2224-2708}
    \gdef\@societyowner{}
}
\DeclareOption{jtaer}{%
    \gdef\@journal{jtaer}
    \gdef\@journalfull{Journal of Theoretical and Applied Electronic Commerce Research}
    \gdef\@journalshort{J. Theor. Appl. Electron. Commer. Res.}
    \gdef\@doiabbr{jtaer}
    \gdef\@ISSN{0718-1876}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jvd}{%
    \gdef\@journal{jvd}
    \gdef\@journalfull{Journal of Vascular Diseases}
    \gdef\@journalshort{J. Vasc. Dis.}
    \gdef\@doiabbr{jvd}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{jzbg}{%
    \gdef\@journal{jzbg}
    \gdef\@journalfull{Journal of Zoological and Botanical Gardens}
    \gdef\@journalshort{J. Zool. Bot. Gard.}
    \gdef\@doiabbr{jzbg}
    \gdef\@ISSN{2673-5636}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
%\DeclareOption{kidney}{%
%	\gdef\@journal{kidney}
%	\gdef\@journalfull{}
%	\gdef\@journalshort{}
%	\gdef\@doiabbr{}
%	\gdef\@ISSN{}
%	\gdef\@continuouspages{yes}
%	\gdef\@societyowner{}
%}
\DeclareOption{kidneydial}{%
    \gdef\@journal{kidneydial}
    \gdef\@journalfull{Kidney and Dialysis}
    \gdef\@journalshort{Kidney Dial.}
    \gdef\@doiabbr{kidneydial}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{kinasesphosphatases}{%
    \gdef\@journal{kinasesphosphatases}
    \gdef\@journalfull{Kinases and Phosphatases}
    \gdef\@journalshort{Kinases Phosphatases}
    \gdef\@doiabbr{kinasesphosphatases}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{knowledge}{%
    \gdef\@journal{knowledge}
    \gdef\@journalfull{Knowledge}
    \gdef\@journalshort{Knowledge}
    \gdef\@doiabbr{knowledge}
    \gdef\@ISSN{2673-9585}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{labmed}{%
    \gdef\@journal{labmed}
    \gdef\@journalfull{LabMed}
    \gdef\@journalshort{LabMed}
    \gdef\@doiabbr{labmed}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{laboratories}{%
    \gdef\@journal{laboratories}
    \gdef\@journalfull{Laboratories}
    \gdef\@journalshort{Laboratories}
    \gdef\@doiabbr{laboratories}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{land}{%
    \gdef\@journal{land}
    \gdef\@journalfull{Land}
    \gdef\@journalshort{Land}
    \gdef\@doiabbr{land}
    \gdef\@ISSN{2073-445X}
    \gdef\@societyowner{}
}
\DeclareOption{languages}{%
    \gdef\@journal{languages}
    \gdef\@journalfull{Languages}
    \gdef\@journalshort{Languages}
    \gdef\@doiabbr{languages}
    \gdef\@ISSN{2226-471X}
    \gdef\@societyowner{}
}
\DeclareOption{laws}{%
    \gdef\@journal{laws}
    \gdef\@journalfull{Laws}
    \gdef\@journalshort{Laws}
    \gdef\@doiabbr{laws}
    \gdef\@ISSN{2075-471X}
    \gdef\@societyowner{}
}
\DeclareOption{life}{%
    \gdef\@journal{life}
    \gdef\@journalfull{Life}
    \gdef\@journalshort{Life}
    \gdef\@doiabbr{life}
    \gdef\@ISSN{2075-1729}
    \gdef\@societyowner{}
}
\DeclareOption{lights}{%
    \gdef\@journal{lights}
    \gdef\@journalfull{Lights}
    \gdef\@journalshort{Lights}
    \gdef\@doiabbr{lights}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{limnolrev}{%
    \gdef\@journal{limnolrev}
    \gdef\@journalfull{Limnological Review}
    \gdef\@journalshort{Limnol. Rev.}
    \gdef\@doiabbr{limnolrev}
    \gdef\@ISSN{2300-7575}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{lipidology}{%
    \gdef\@journal{lipidology}
    \gdef\@journalfull{Lipidology}
    \gdef\@journalshort{Lipidology}
    \gdef\@doiabbr{lipidology}
    \gdef\@ISSN{2813-7086}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{liquids}{%
    \gdef\@journal{liquids}
    \gdef\@journalfull{Liquids}
    \gdef\@journalshort{Liquids}
    \gdef\@doiabbr{liquids}
    \gdef\@ISSN{2673-8015}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{literature}{%
    \gdef\@journal{literature}
    \gdef\@journalfull{Literature}
    \gdef\@journalshort{Literature}
    \gdef\@doiabbr{literature}
    \gdef\@ISSN{2410-9789}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{livers}{%
    \gdef\@journal{livers}
    \gdef\@journalfull{Livers}
    \gdef\@journalshort{Livers}
    \gdef\@doiabbr{livers}
    \gdef\@ISSN{2673-4389}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{logics}{%
    \gdef\@journal{logics}
    \gdef\@journalfull{Logics}
    \gdef\@journalshort{Logics}
    \gdef\@doiabbr{logics}
    \gdef\@ISSN{2813-0405}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{logistics}{%
    \gdef\@journal{logistics}
    \gdef\@journalfull{Logistics}
    \gdef\@journalshort{Logistics}
    \gdef\@doiabbr{logistics}
    \gdef\@ISSN{2305-6290}
    \gdef\@societyowner{}
}
\DeclareOption{lubricants}{%
    \gdef\@journal{lubricants}
    \gdef\@journalfull{Lubricants}
    \gdef\@journalshort{Lubricants}
    \gdef\@doiabbr{lubricants}
    \gdef\@ISSN{2075-4442}
    \gdef\@societyowner{}
}
\DeclareOption{lymphatics}{%
    \gdef\@journal{lymphatics}
    \gdef\@journalfull{Lymphatics}
    \gdef\@journalshort{Lymphatics}
    \gdef\@doiabbr{lymphatics}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{machines}{%
    \gdef\@journal{machines}
    \gdef\@journalfull{Machines}
    \gdef\@journalshort{Machines}
    \gdef\@doiabbr{machines}
    \gdef\@ISSN{2075-1702}
    \gdef\@societyowner{}
}
\DeclareOption{macromol}{%
    \gdef\@journal{macromol}
    \gdef\@journalfull{Macromol}
    \gdef\@journalshort{Macromol}
    \gdef\@doiabbr{macromol}
    \gdef\@ISSN{2673-6209}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{magnetism}{%
    \gdef\@journal{magnetism}
    \gdef\@journalfull{Magnetism}
    \gdef\@journalshort{Magnetism}
    \gdef\@doiabbr{magnetism}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{magnetochemistry}{%
    \gdef\@journal{magnetochemistry}
    \gdef\@journalfull{Magnetochemistry}
    \gdef\@journalshort{Magnetochemistry}
    \gdef\@doiabbr{magnetochemistry}
    \gdef\@ISSN{2312-7481}
    \gdef\@societyowner{}
}
\DeclareOption{make}{%
    \gdef\@journal{make}
    \gdef\@journalfull{Machine Learning and Knowledge Extraction}
    \gdef\@journalshort{Mach. Learn. Knowl. Extr.}
    \gdef\@doiabbr{make}
    \gdef\@ISSN{2504-4990}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{marinedrugs}{%
    \gdef\@journal{marinedrugs}
    \gdef\@journalfull{Marine Drugs}
    \gdef\@journalshort{Mar. Drugs}
    \gdef\@doiabbr{md}
    \gdef\@ISSN{1660-3397}
    \gdef\@societyowner{}
}
\DeclareOption{materials}{%
    \gdef\@journal{materials}
    \gdef\@journalfull{Materials}
    \gdef\@journalshort{Materials}
    \gdef\@doiabbr{ma}
    \gdef\@ISSN{1996-1944}
    \gdef\@societyowner{}
}
\DeclareOption{materproc}{%
    \gdef\@journal{materproc}
    \gdef\@journalfull{Materials Proceedings}
    \gdef\@journalshort{Mater. Proc.}
    \gdef\@doiabbr{materproc}
    \gdef\@ISSN{2673-4605}
    \gdef\@societyowner{}
}
\DeclareOption{mathematics}{%
    \gdef\@journal{mathematics}
    \gdef\@journalfull{Mathematics}
    \gdef\@journalshort{Mathematics}
    \gdef\@doiabbr{math}
    \gdef\@ISSN{2227-7390}
    \gdef\@societyowner{}
}
\DeclareOption{mca}{%
    \gdef\@journal{mca}
    \gdef\@journalfull{Mathematical and Computational Applications}
    \gdef\@journalshort{Math. Comput. Appl.}
    \gdef\@doiabbr{mca}
    \gdef\@ISSN{2297-8747}
    \gdef\@societyowner{}
}
\DeclareOption{measurements}{%
    \gdef\@journal{measurements}
    \gdef\@journalfull{Measurements}
    \gdef\@journalshort{Measurements}
    \gdef\@doiabbr{measurements}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{medicina}{%
    \gdef\@journal{medicina}
    \gdef\@journalfull{Medicina}
    \gdef\@journalshort{Medicina}
    \gdef\@doiabbr{medicina}
    \gdef\@ISSN{1648-9144}
    \gdef\@societyowner{Lithuanian University of Health Sciences}
}
\DeclareOption{medicines}{%
    \gdef\@journal{medicines}
    \gdef\@journalfull{Medicines}
    \gdef\@journalshort{Medicines}
    \gdef\@doiabbr{medicines}
    \gdef\@ISSN{2305-6320}
    \gdef\@societyowner{}
}
\DeclareOption{medsci}{%
    \gdef\@journal{medsci}
    \gdef\@journalfull{Medical Sciences}
    \gdef\@journalshort{Med. Sci.}
    \gdef\@doiabbr{medsci}
    \gdef\@ISSN{2076-3271}
    \gdef\@societyowner{}
}
\DeclareOption{membranes}{%
    \gdef\@journal{membranes}
    \gdef\@journalfull{Membranes}
    \gdef\@journalshort{Membranes}
    \gdef\@doiabbr{membranes}
    \gdef\@ISSN{2077-0375}
    \gdef\@societyowner{}
}
\DeclareOption{merits}{%
    \gdef\@journal{merits}
    \gdef\@journalfull{Merits}
    \gdef\@journalshort{Merits}
    \gdef\@doiabbr{merits}
    \gdef\@ISSN{2673-8104}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{metabolites}{%
    \gdef\@journal{metabolites}
    \gdef\@journalfull{Metabolites}
    \gdef\@journalshort{Metabolites}
    \gdef\@doiabbr{metabo}
    \gdef\@ISSN{2218-1989}
    \gdef\@societyowner{}
}
\DeclareOption{metals}{%
    \gdef\@journal{metals}
    \gdef\@journalfull{Metals}
    \gdef\@journalshort{Metals}
    \gdef\@doiabbr{met}
    \gdef\@ISSN{2075-4701}
    \gdef\@societyowner{}
}
\DeclareOption{meteorology}{%
    \gdef\@journal{meteorology}
    \gdef\@journalfull{Meteorology}
    \gdef\@journalshort{Meteorology}
    \gdef\@doiabbr{meteorology}
    \gdef\@ISSN{2674-0494}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{methane}{%
    \gdef\@journal{methane}
    \gdef\@journalfull{Methane}
    \gdef\@journalshort{Methane}
    \gdef\@doiabbr{methane}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{metrics}{%
    \gdef\@journal{metrics}
    \gdef\@journalfull{Metrics}
    \gdef\@journalshort{Metrics}
    \gdef\@doiabbr{metrics}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{metrology}{%
    \gdef\@journal{metrology}
    \gdef\@journalfull{Metrology}
    \gdef\@journalshort{Metrology}
    \gdef\@doiabbr{metrology}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{micro}{%
    \gdef\@journal{micro}
    \gdef\@journalfull{Micro}
    \gdef\@journalshort{Micro}
    \gdef\@doiabbr{micro}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{microarrays}{%
    \gdef\@journal{microarrays}
    \gdef\@journalfull{Microarrays}
    \gdef\@journalshort{Microarrays}
    \gdef\@doiabbr{microarrays}
    \gdef\@ISSN{2076-3905}
    \gdef\@societyowner{}
}
\DeclareOption{microbiolres}{%
    \gdef\@journal{microbiolres}
    \gdef\@journalfull{Microbiology Research}
    \gdef\@journalshort{Microbiol. Res.}
    \gdef\@doiabbr{microbiolres}
    \gdef\@ISSN{2036-7481}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{microelectronics}{%
    \gdef\@journal{microelectronics}
    \gdef\@journalfull{Microelectronics}
    \gdef\@journalshort{Microelectronics}
    \gdef\@doiabbr{microelectronics}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{micromachines}{%
    \gdef\@journal{micromachines}
    \gdef\@journalfull{Micromachines}
    \gdef\@journalshort{Micromachines}
    \gdef\@doiabbr{mi}
    \gdef\@ISSN{2072-666X}
    \gdef\@societyowner{}
}
\DeclareOption{microorganisms}{%
    \gdef\@journal{microorganisms}
    \gdef\@journalfull{Microorganisms}
    \gdef\@journalshort{Microorganisms}
    \gdef\@doiabbr{microorganisms}
    \gdef\@ISSN{2076-2607}
    \gdef\@societyowner{}
}
\DeclareOption{microplastics}{%
    \gdef\@journal{microplastics}
    \gdef\@journalfull{Microplastics}
    \gdef\@journalshort{Microplastics}
    \gdef\@doiabbr{microplastics}
    \gdef\@ISSN{2673-8929}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{microwave}{%
    \gdef\@journal{microwave}
    \gdef\@journalfull{Microwave}
    \gdef\@journalshort{Microwave}
    \gdef\@doiabbr{microwave}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{minerals}{%
    \gdef\@journal{minerals}
    \gdef\@journalfull{Minerals}
    \gdef\@journalshort{Minerals}
    \gdef\@doiabbr{min}
    \gdef\@ISSN{2075-163X}
    \gdef\@societyowner{}
}
\DeclareOption{mining}{%
    \gdef\@journal{mining}
    \gdef\@journalfull{Mining}
    \gdef\@journalshort{Mining}
    \gdef\@doiabbr{mining}
    \gdef\@ISSN{2673-6489}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{mmphys}{%
    \gdef\@journal{mmphys}
    \gdef\@journalfull{Modern Mathematical Physics}
    \gdef\@journalshort{Mod. Math. Phys.}
    \gdef\@doiabbr{mmphys}\gdef\@ISSN{3042-5034}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{modelling}{%
    \gdef\@journal{modelling}
    \gdef\@journalfull{Modelling}
    \gdef\@journalshort{Modelling}
    \gdef\@doiabbr{modelling}
    \gdef\@ISSN{2673-3951}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{molbank}{%
    \gdef\@journal{molbank}
    \gdef\@journalfull{Molbank}
    \gdef\@journalshort{Molbank}
    \gdef\@doiabbr{M}
    \gdef\@ISSN{1422-8599}
    \gdef\@societyowner{}
}
\DeclareOption{molecules}{%
    \gdef\@journal{molecules}
    \gdef\@journalfull{Molecules}
    \gdef\@journalshort{Molecules}
    \gdef\@doiabbr{molecules}
    \gdef\@ISSN{1420-3049}
    \gdef\@societyowner{}
}
\DeclareOption{mps}{%
    \gdef\@journal{mps}
    \gdef\@journalfull{Methods and Protocols}
    \gdef\@journalshort{Methods Protoc.}
    \gdef\@doiabbr{mps}
    \gdef\@ISSN{2409-9279}
    \gdef\@societyowner{}
}
\DeclareOption{msf}{%
    \gdef\@journal{msf}
    \gdef\@journalfull{Medical Sciences Forum}
    \gdef\@journalshort{Med. Sci. Forum}
    \gdef\@doiabbr{msf}
    \gdef\@ISSN{2673-9992}
    \gdef\@societyowner{}
}
\DeclareOption{mti}{%
    \gdef\@journal{mti}
    \gdef\@journalfull{Multimodal Technologies and Interaction}
    \gdef\@journalshort{Multimodal Technol. Interact.}
    \gdef\@doiabbr{mti}
    \gdef\@ISSN{2414-4088}
    \gdef\@societyowner{}
}
\DeclareOption{multimedia}{%
    \gdef\@journal{multimedia}
    \gdef\@journalfull{Multimedia}
    \gdef\@journalshort{Multimedia}
    \gdef\@doiabbr{multimedia}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{muscles}{%
    \gdef\@journal{muscles}
    \gdef\@journalfull{Muscles}
    \gdef\@journalshort{Muscles}
    \gdef\@doiabbr{muscles}
    \gdef\@ISSN{2813-0413}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{nanoenergyadv}{%
    \gdef\@journal{nanoenergyadv}
    \gdef\@journalfull{Nanoenergy Advances}
    \gdef\@journalshort{Nanoenergy Adv.}
    \gdef\@doiabbr{nanoenergyadv}
    \gdef\@ISSN{2673-706X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{nanomanufacturing}{%
    \gdef\@journal{nanomanufacturing}
    \gdef\@journalfull{Nanomanufacturing}
    \gdef\@journalshort{Nanomanufacturing}
    \gdef\@doiabbr{nanomanufacturing}
    \gdef\@ISSN{2673-687X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{nanomaterials}{%
    \gdef\@journal{nanomaterials}
    \gdef\@journalfull{Nanomaterials}
    \gdef\@journalshort{Nanomaterials}
    \gdef\@doiabbr{nano}
    \gdef\@ISSN{2079-4991}
    \gdef\@societyowner{}
}
\DeclareOption{ncrna}{%
    \gdef\@journal{ncrna}
    \gdef\@journalfull{Non-Coding RNA}
    \gdef\@journalshort{Non-Coding RNA}
    \gdef\@doiabbr{ncrna}
    \gdef\@ISSN{2311-553X}
    \gdef\@societyowner{}
}
\DeclareOption{ndt}{%
    \gdef\@journal{ndt}
    \gdef\@journalfull{NDT}
    \gdef\@journalshort{NDT}
    \gdef\@doiabbr{ndt}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{network}{%
    \gdef\@journal{network}
    \gdef\@journalfull{Network}
    \gdef\@journalshort{Network}
    \gdef\@doiabbr{network}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{neuroglia}{%
    \gdef\@journal{neuroglia}
    \gdef\@journalfull{Neuroglia}
    \gdef\@journalshort{Neuroglia}
    \gdef\@doiabbr{neuroglia}
    \gdef\@ISSN{2571-6980}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{neurolint}{%
    \gdef\@journal{neurolint}
    \gdef\@journalfull{Neurology International}
    \gdef\@journalshort{Neurol. Int.}
    \gdef\@doiabbr{neurolint}
    \gdef\@ISSN{2035-8377}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{neurosci}{%
    \gdef\@journal{neurosci}
    \gdef\@journalfull{NeuroSci}
    \gdef\@journalshort{NeuroSci}
    \gdef\@doiabbr{neurosci}
    \gdef\@ISSN{2673-4087}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{nitrogen}{%
    \gdef\@journal{nitrogen}
    \gdef\@journalfull{Nitrogen}
    \gdef\@journalshort{Nitrogen}
    \gdef\@doiabbr{nitrogen}
    \gdef\@ISSN{2504-3129}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{notspecified}{%
    \gdef\@journal{notspecified}
    \gdef\@journalfull{Journal Not Specified}
    \gdef\@journalshort{Journal Not Specified}
    \gdef\@doiabbr{}
    \gdef\@ISSN{}
    \gdef\@societyowner{}
}
\DeclareOption{nri}{%
    \gdef\@journal{nri}
    \gdef\@journalfull{Natural Resources Informatics}
    \gdef\@journalshort{Nat. Resour. Inform.}
    \gdef\@doiabbr{nri}
    \gdef\@ISSN{2673-981X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{nursrep}{%
    \gdef\@journal{nursrep}
    \gdef\@journalfull{Nursing Reports}
    \gdef\@journalshort{Nurs. Rep.}
    \gdef\@doiabbr{nursrep}
    \gdef\@ISSN{2039-4403}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{nutraceuticals}{%
    \gdef\@journal{nutraceuticals}
    \gdef\@journalfull{Nutraceuticals}
    \gdef\@journalshort{Nutraceuticals}
    \gdef\@doiabbr{nutraceuticals}
    \gdef\@ISSN{1661-3821}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{nutrients}{%
    \gdef\@journal{nutrients}
    \gdef\@journalfull{Nutrients}
    \gdef\@journalshort{Nutrients}
    \gdef\@doiabbr{nu}
    \gdef\@ISSN{2072-6643}
    \gdef\@societyowner{}
}
\DeclareOption{obesities}{%
    \gdef\@journal{obesities}
    \gdef\@journalfull{Obesities}
    \gdef\@journalshort{Obesities}
    \gdef\@doiabbr{obesities}
    \gdef\@ISSN{2673-4168}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{oceans}{%
    \gdef\@journal{oceans}
    \gdef\@journalfull{Oceans}
    \gdef\@journalshort{Oceans}
    \gdef\@doiabbr{oceans}
    \gdef\@ISSN{2673-1924}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{ohbm}{%
    \gdef\@journal{ohbm}
    \gdef\@journalfull{Journal of Otorhinolaryngology, Hearing and Balance Medicine}
    \gdef\@journalshort{J. Otorhinolaryngol. Hear. Balance Med.}
    \gdef\@doiabbr{ohbm}
    \gdef\@ISSN{2504-463X}
    \gdef\@societyowner{}
}
\DeclareOption{onco}{%
    \gdef\@journal{onco}
    \gdef\@journalfull{Onco}
    \gdef\@journalshort{Onco}
    \gdef\@doiabbr{onco}
    \gdef\@ISSN{2673-7523}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
%\DeclareOption{oncopathology}{%
%	\gdef\@journal{oncopathology}
%	\gdef\@journalfull{}
%	\gdef\@journalshort{}
%	\gdef\@doiabbr{}
%	\gdef\@ISSN{}
%	\gdef\@continuouspages{yes}
%	\gdef\@societyowner{}
%}
\DeclareOption{optics}{%
    \gdef\@journal{optics}
    \gdef\@journalfull{Optics}
    \gdef\@journalshort{Optics}
    \gdef\@doiabbr{opt}
    \gdef\@ISSN{2673-3269}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{oral}{%
    \gdef\@journal{oral}
    \gdef\@journalfull{Oral}
    \gdef\@journalshort{Oral}
    \gdef\@doiabbr{oral}
    \gdef\@ISSN{2673-6373}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{organics}{%
    \gdef\@journal{organics}
    \gdef\@journalfull{Organics}
    \gdef\@journalshort{Organics}
    \gdef\@doiabbr{org}
    \gdef\@ISSN{2673-401X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{organoids}{%
    \gdef\@journal{organoids}
    \gdef\@journalfull{Organoids}
    \gdef\@journalshort{Organoids}
    \gdef\@doiabbr{organoids}
    \gdef\@ISSN{2674-1172}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{osteology}{%
    \gdef\@journal{osteology}
    \gdef\@journalfull{Osteology}
    \gdef\@journalshort{Osteology}
    \gdef\@doiabbr{osteology}
    \gdef\@ISSN{2673-4036}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{oxygen}{%
    \gdef\@journal{oxygen}
    \gdef\@journalfull{Oxygen}
    \gdef\@journalshort{Oxygen}
    \gdef\@doiabbr{oxygen}
    \gdef\@ISSN{2673-9801}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{parasites}{%
    \gdef\@journal{parasites}
    \gdef\@journalfull{Parasites}
    \gdef\@journalshort{Parasites}
    \gdef\@doiabbr{parasites}
    \gdef\@ISSN{2673-5946}
    \gdef\@societyowner{}
}
\DeclareOption{parasitologia}{%
    \gdef\@journal{parasitologia}
    \gdef\@journalfull{Parasitologia}
    \gdef\@journalshort{Parasitologia}
    \gdef\@doiabbr{parasitologia}
    \gdef\@ISSN{2673-6772}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{particles}{%
    \gdef\@journal{particles}
    \gdef\@journalfull{Particles}
    \gdef\@journalshort{Particles}
    \gdef\@doiabbr{particles}
    \gdef\@ISSN{2571-712X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{pathogens}{%
    \gdef\@journal{pathogens}
    \gdef\@journalfull{Pathogens}
    \gdef\@journalshort{Pathogens}
    \gdef\@doiabbr{pathogens}
    \gdef\@ISSN{2076-0817}
    \gdef\@societyowner{}
}
\DeclareOption{pathophysiology}{%
    \gdef\@journal{pathophysiology}
    \gdef\@journalfull{Pathophysiology}
    \gdef\@journalshort{Pathophysiology}
    \gdef\@doiabbr{pathophysiology}
    \gdef\@ISSN{0928-4680}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{pediatrrep}{%
    \gdef\@journal{pediatrrep}
    \gdef\@journalfull{Pediatric Reports}
    \gdef\@journalshort{Pediatr. Rep.}
    \gdef\@doiabbr{pediatric}
    \gdef\@ISSN{2036-7503}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{pets}{%
    \gdef\@journal{pets}
    \gdef\@journalfull{Pets}
    \gdef\@journalshort{Pets}
    \gdef\@doiabbr{pets}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{pharmaceuticals}{%
    \gdef\@journal{pharmaceuticals}
    \gdef\@journalfull{Pharmaceuticals}
    \gdef\@journalshort{Pharmaceuticals}
    \gdef\@doiabbr{ph}
    \gdef\@ISSN{1424-8247}
    \gdef\@societyowner{}
}
\DeclareOption{pharmaceutics}{%
    \gdef\@journal{pharmaceutics}
    \gdef\@journalfull{Pharmaceutics}
    \gdef\@journalshort{Pharmaceutics}
    \gdef\@doiabbr{pharmaceutics}
    \gdef\@ISSN{1999-4923}
    \gdef\@societyowner{}
}
\DeclareOption{pharmacoepidemiology}{%
    \gdef\@journal{pharmacoepidemiology}
    \gdef\@journalfull{Pharmacoepidemiology}
    \gdef\@journalshort{Pharmacoepidemiology}
    \gdef\@doiabbr{pharma}
    \gdef\@ISSN{2813-0618}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{pharmacy}{%
    \gdef\@journal{pharmacy}
    \gdef\@journalfull{Pharmacy}
    \gdef\@journalshort{Pharmacy}
    \gdef\@doiabbr{pharmacy}
    \gdef\@ISSN{2226-4787}
    \gdef\@societyowner{}
}
\DeclareOption{philosophies}{%
    \gdef\@journal{philosophies}
    \gdef\@journalfull{Philosophies}
    \gdef\@journalshort{Philosophies}
    \gdef\@doiabbr{philosophies}
    \gdef\@ISSN{2409-9287}
    \gdef\@societyowner{}
}
\DeclareOption{photochem}{%
    \gdef\@journal{photochem}
    \gdef\@journalfull{Photochem}
    \gdef\@journalshort{Photochem}
    \gdef\@doiabbr{photochem}
    \gdef\@ISSN{2673-7256}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{photonics}{%
    \gdef\@journal{photonics}
    \gdef\@journalfull{Photonics}
    \gdef\@journalshort{Photonics}
    \gdef\@doiabbr{photonics}
    \gdef\@ISSN{2304-6732}
    \gdef\@societyowner{}
}
\DeclareOption{phycology}{%
    \gdef\@journal{phycology}
    \gdef\@journalfull{Phycology}
    \gdef\@journalshort{Phycology}
    \gdef\@doiabbr{phycology}
    \gdef\@ISSN{2673-9410}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{physchem}{%
    \gdef\@journal{physchem}
    \gdef\@journalfull{Physchem}
    \gdef\@journalshort{Physchem}
    \gdef\@doiabbr{physchem}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{physics}{%
    \gdef\@journal{physics}
    \gdef\@journalfull{Physics}
    \gdef\@journalshort{Physics}
    \gdef\@doiabbr{physics}
    \gdef\@ISSN{2624-8174}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{physiologia}{%
    \gdef\@journal{physiologia}
    \gdef\@journalfull{Physiologia}
    \gdef\@journalshort{Physiologia}
    \gdef\@doiabbr{physiologia}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{plants}{%
    \gdef\@journal{plants}
    \gdef\@journalfull{Plants}
    \gdef\@journalshort{Plants}
    \gdef\@doiabbr{plants}
    \gdef\@ISSN{2223-7747}
    \gdef\@societyowner{}
}
\DeclareOption{plasma}{%
    \gdef\@journal{plasma}
    \gdef\@journalfull{Plasma}
    \gdef\@journalshort{Plasma}
    \gdef\@doiabbr{plasma}
    \gdef\@ISSN{2571-6182}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{platforms}{%
    \gdef\@journal{platforms}
    \gdef\@journalfull{Platforms}
    \gdef\@journalshort{Platforms}
    \gdef\@doiabbr{platforms}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{pollutants}{%
    \gdef\@journal{pollutants}
    \gdef\@journalfull{Pollutants}
    \gdef\@journalshort{Pollutants}
    \gdef\@doiabbr{pollutants}
    \gdef\@ISSN{2673-4672}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{polymers}{%
    \gdef\@journal{polymers}
    \gdef\@journalfull{Polymers}
    \gdef\@journalshort{Polymers}
    \gdef\@doiabbr{polym}
    \gdef\@ISSN{2073-4360}
    \gdef\@societyowner{}
}
\DeclareOption{polysaccharides}{%
    \gdef\@journal{polysaccharides}
    \gdef\@journalfull{Polysaccharides}
    \gdef\@journalshort{Polysaccharides}
    \gdef\@doiabbr{polysaccharides}
    \gdef\@ISSN{2673-4176}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{populations}{%
    \gdef\@journal{populations}
    \gdef\@journalfull{Populations}
    \gdef\@journalshort{Populations}
    \gdef\@doiabbr{populations}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{poultry}{%
    \gdef\@journal{poultry}
    \gdef\@journalfull{Poultry}
    \gdef\@journalshort{Poultry}
    \gdef\@doiabbr{poultry}
    \gdef\@ISSN{2674-1164}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{powders}{%
    \gdef\@journal{powders}
    \gdef\@journalfull{Powders}
    \gdef\@journalshort{Powders}
    \gdef\@doiabbr{powders}
    \gdef\@ISSN{2674-0516}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
% \DeclareOption{preprints}{%
% 	\gdef\@journal{preprints}
% 	\gdef\@journalfull{Preprints}
% 	\gdef\@journalshort{Preprints}
% 	\gdef\@doiabbr{}
% 	\gdef\@ISSN{}
% 	\gdef\@societyowner{}
% }
\DeclareOption{preprints}{%
    \gdef\@journal{preprints}
    \gdef\@journalfull{arXiv}
    \gdef\@journalshort{arXiv}
    \gdef\@doiabbr{}
    \gdef\@ISSN{}
    \gdef\@societyowner{}
}
\DeclareOption{proceedings}{%
    \gdef\@journal{proceedings}
    \gdef\@journalfull{Proceedings}
    \gdef\@journalshort{Proceedings}
    \gdef\@doiabbr{proceedings}
    \gdef\@ISSN{2504-3900}
    \gdef\@societyowner{}
}
\DeclareOption{processes}{%
    \gdef\@journal{processes}
    \gdef\@journalfull{Processes}
    \gdef\@journalshort{Processes}
    \gdef\@doiabbr{pr}
    \gdef\@ISSN{2227-9717}
    \gdef\@societyowner{}
}
\DeclareOption{prosthesis}{%
    \gdef\@journal{prosthesis}
    \gdef\@journalfull{Prosthesis}
    \gdef\@journalshort{Prosthesis}
    \gdef\@doiabbr{prosthesis}
    \gdef\@ISSN{2673-1592}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{proteomes}{%
    \gdef\@journal{proteomes}
    \gdef\@journalfull{Proteomes}
    \gdef\@journalshort{Proteomes}
    \gdef\@doiabbr{proteomes}
    \gdef\@ISSN{2227-7382}
    \gdef\@societyowner{}
}
\DeclareOption{psf}{%
    \gdef\@journal{psf}
    \gdef\@journalfull{Physical Sciences Forum}
    \gdef\@journalshort{Phys. Sci. Forum}
    \gdef\@doiabbr{psf}
    \gdef\@ISSN{2673-9984}
    \gdef\@societyowner{}
}
%\DeclareOption{psych}{%
%	\gdef\@journal{psych}
%	\gdef\@journalfull{Psych}
%   \gdef\@journalshort{Psych}
%	\gdef\@doiabbr{psych}
%	\gdef\@ISSN{2624-8611}
%	\gdef\@continuouspages{yes}
%	\gdef\@societyowner{}
%}
\DeclareOption{psychiatryint}{%
    \gdef\@journal{psychiatryint}
    \gdef\@journalfull{Psychiatry International}
    \gdef\@journalshort{Psychiatry Int.}
    \gdef\@doiabbr{psychiatryint}
    \gdef\@ISSN{2673-5318}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{psychoactives}{%
    \gdef\@journal{psychoactives}
    \gdef\@journalfull{Psychoactives}
    \gdef\@journalshort{Psychoactives}
    \gdef\@doiabbr{psychoactives}
    \gdef\@ISSN{2813-1851}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{psycholint}{%
    \gdef\@journal{psycholint}
    \gdef\@journalfull{Psychology International}
    \gdef\@journalshort{Psychol. Int.}
    \gdef\@doiabbr{psycholint}
    \gdef\@ISSN{2813-9844}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{publications}{%
    \gdef\@journal{publications}
    \gdef\@journalfull{Publications}
    \gdef\@journalshort{Publications}
    \gdef\@doiabbr{publications}
    \gdef\@ISSN{2304-6775}
    \gdef\@societyowner{}
}
\DeclareOption{purification}{%
    \gdef\@journal{purification}
    \gdef\@journalfull{Purification}
    \gdef\@journalshort{Purification}
    \gdef\@doiabbr{purification}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{quantumrep}{%
    \gdef\@journal{quantumrep}
    \gdef\@journalfull{Quantum Reports}
    \gdef\@journalshort{Quantum Rep.}
    \gdef\@doiabbr{quantum}
    \gdef\@ISSN{2624-960X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{quaternary}{%
    \gdef\@journal{quaternary}
    \gdef\@journalfull{Quaternary}
    \gdef\@journalshort{Quaternary}
    \gdef\@doiabbr{quat}
    \gdef\@ISSN{2571-550X}
    \gdef\@societyowner{}
}
\DeclareOption{qubs}{%
    \gdef\@journal{qubs}
    \gdef\@journalfull{Quantum Beam Science}
    \gdef\@journalshort{Quantum Beam Sci.}
    \gdef\@doiabbr{qubs}
    \gdef\@ISSN{2412-382X}
    \gdef\@societyowner{}
}
\DeclareOption{radiation}{%
    \gdef\@journal{radiation}
    \gdef\@journalfull{Radiation}
    \gdef\@journalshort{Radiation}
    \gdef\@doiabbr{radiation}
    \gdef\@ISSN{2673-592X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{reactions}{%
    \gdef\@journal{reactions}
    \gdef\@journalfull{Reactions}
    \gdef\@journalshort{Reactions}
    \gdef\@doiabbr{reactions}
    \gdef\@ISSN{2624-781X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{realestate}{%
    \gdef\@journal{realestate}
    \gdef\@journalfull{Real Estate}
    \gdef\@journalshort{Real Estate}
    \gdef\@doiabbr{realestate}
    \gdef\@ISSN{2813-8090}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{receptors}{%
    \gdef\@journal{receptors}
    \gdef\@journalfull{Receptors}
    \gdef\@journalshort{Receptors}
    \gdef\@doiabbr{receptors}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{recycling}{%
    \gdef\@journal{recycling}
    \gdef\@journalfull{Recycling}
    \gdef\@journalshort{Recycling}
    \gdef\@doiabbr{recycling}
    \gdef\@ISSN{2313-4321}
    \gdef\@societyowner{}
}
\DeclareOption{regeneration}{%
    \gdef\@journal{regeneration}
    \gdef\@journalfull{Regeneration}
    \gdef\@journalshort{Regeneration}
    \gdef\@doiabbr{regeneration}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{religions}{%
    \gdef\@journal{religions}
    \gdef\@journalfull{Religions}
    \gdef\@journalshort{Religions}
    \gdef\@doiabbr{rel}
    \gdef\@ISSN{2077-1444}
    \gdef\@societyowner{}
}
\DeclareOption{remotesensing}{%
    \gdef\@journal{remotesensing}
    \gdef\@journalfull{Remote Sensing}
    \gdef\@journalshort{Remote Sens.}
    \gdef\@doiabbr{rs}
    \gdef\@ISSN{2072-4292}
    \gdef\@societyowner{}
}
\DeclareOption{reports}{%
    \gdef\@journal{reports}
    \gdef\@journalfull{Reports}
    \gdef\@journalshort{Reports}
    \gdef\@doiabbr{reports}
    \gdef\@ISSN{2571-841X}
    \gdef\@societyowner{}
}
\DeclareOption{reprodmed}{%
    \gdef\@journal{reprodmed}
    \gdef\@journalfull{Reproductive Medicine}
    \gdef\@journalshort{Reprod. Med.}
    \gdef\@doiabbr{reprodmed}
    \gdef\@ISSN{2673-3897}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{resources}{%
    \gdef\@journal{resources}
    \gdef\@journalfull{Resources}
    \gdef\@journalshort{Resources}
    \gdef\@doiabbr{resources}
    \gdef\@ISSN{2079-9276}
    \gdef\@societyowner{}
}
\DeclareOption{rheumato}{%
    \gdef\@journal{rheumato}
    \gdef\@journalfull{Rheumato}
    \gdef\@journalshort{Rheumato}
    \gdef\@doiabbr{rheumato}
    \gdef\@ISSN{2674-0621}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{risks}{%
    \gdef\@journal{risks}
    \gdef\@journalfull{Risks}
    \gdef\@journalshort{Risks}
    \gdef\@doiabbr{risks}
    \gdef\@ISSN{2227-9091}
    \gdef\@societyowner{}
}
\DeclareOption{robotics}{%
    \gdef\@journal{robotics}
    \gdef\@journalfull{Robotics}
    \gdef\@journalshort{Robotics}
    \gdef\@doiabbr{robotics}
    \gdef\@ISSN{2218-6581}
    \gdef\@societyowner{}
}
\DeclareOption{rsee}{%
    \gdef\@journal{rsee}
    \gdef\@journalfull{Regional Science and Environmental Economics}
    \gdef\@journalshort{Reg. Sci. Environ. Econ.}
    \gdef\@doiabbr{rsee}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{ruminants}{%
    \gdef\@journal{ruminants}
    \gdef\@journalfull{Ruminants}
    \gdef\@journalshort{Ruminants}
    \gdef\@doiabbr{ruminants}
    \gdef\@ISSN{2673-933X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{safety}{%
    \gdef\@journal{safety}
    \gdef\@journalfull{Safety}
    \gdef\@journalshort{Safety}
    \gdef\@doiabbr{safety}
    \gdef\@ISSN{2313-576X}
    \gdef\@societyowner{}
}
\DeclareOption{sci}{%
    \gdef\@journal{sci}
    \gdef\@journalfull{Sci}
    \gdef\@journalshort{Sci}
    \gdef\@doiabbr{sci}
    \gdef\@ISSN{2413-4155}
    \gdef\@societyowner{}
}
\DeclareOption{scipharm}{%
\gdef\@journal{scipharm}
\gdef\@journalfull{Scientia Pharmaceutica}
\gdef\@journalshort{Sci. Pharm.}
\gdef\@doiabbr{scipharm}
\gdef\@ISSN{2218-0532}
\gdef\@societyowner{\"{O}sterreichische Pharmazeutische Gesellschaft}
}
\DeclareOption{sclerosis}{%
    \gdef\@journal{sclerosis}
    \gdef\@journalfull{Sclerosis}
    \gdef\@journalshort{Sclerosis}
    \gdef\@doiabbr{sclerosis}
    \gdef\@ISSN{2813-3064}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{seeds}{%
    \gdef\@journal{seeds}
    \gdef\@journalfull{Seeds}
    \gdef\@journalshort{Seeds}
    \gdef\@doiabbr{seeds}
    \gdef\@ISSN{2674-1024}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{sensors}{%
    \gdef\@journal{sensors}
    \gdef\@journalfull{Sensors}
    \gdef\@journalshort{Sensors}
    \gdef\@doiabbr{s}
    \gdef\@ISSN{1424-8220}
    \gdef\@societyowner{}
}
\DeclareOption{separations}{%
    \gdef\@journal{separations}
    \gdef\@journalfull{Separations}
    \gdef\@journalshort{Separations}
    \gdef\@doiabbr{separations}
    \gdef\@ISSN{2297-8739}
    \gdef\@societyowner{}
}
\DeclareOption{sexes}{%
    \gdef\@journal{sexes}
    \gdef\@journalfull{Sexes}
    \gdef\@journalshort{Sexes}
    \gdef\@doiabbr{sexes}
    \gdef\@ISSN{2411-5118}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{signals}{%
    \gdef\@journal{signals}
    \gdef\@journalfull{Signals}
    \gdef\@journalshort{Signals}
    \gdef\@doiabbr{signals}
    \gdef\@ISSN{2624-6120}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{sinusitis}{%
    \gdef\@journal{sinusitis}
    \gdef\@journalfull{Sinusitis}
    \gdef\@journalshort{Sinusitis}
    \gdef\@doiabbr{sinusitis}
    \gdef\@ISSN{2309-107X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{siuj}{%
\gdef\@journal{siuj}
\gdef\@journalfull{Soci\'{e}t\'{e} Internationale d'Urologie Journal}
\gdef\@journalshort{Soc. Int. Urol. J.}
\gdef\@doiabbr{siuj}
\gdef\@ISSN{2563-6499}
\gdef\@continuouspages{yes}
\gdef\@societyowner{Soci\'{e}t\'{e} Internationale d'Urologie}
}
\DeclareOption{skins}{%
    \gdef\@journal{skins}
    \gdef\@journalfull{Skins}
    \gdef\@journalshort{Skins}
    \gdef\@doiabbr{skins}
    \gdef\@ISSN{}
    \gdef\@societyowner{}
}
\DeclareOption{smartcities}{%
    \gdef\@journal{smartcities}
    \gdef\@journalfull{Smart Cities}
    \gdef\@journalshort{Smart Cities}
    \gdef\@doiabbr{smartcities}
    \gdef\@ISSN{2624-6511}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{sna}{%
    \gdef\@journal{sna}
    \gdef\@journalfull{Sinusitis and Asthma}
    \gdef\@journalshort{Sinusitis Asthma}
    \gdef\@doiabbr{sna}
    \gdef\@ISSN{2624-7003}
    \gdef\@societyowner{}
}
\DeclareOption{societies}{%
    \gdef\@journal{societies}
    \gdef\@journalfull{Societies}
    \gdef\@journalshort{Societies}
    \gdef\@doiabbr{soc}
    \gdef\@ISSN{2075-4698}
    \gdef\@societyowner{}
}
\DeclareOption{socsci}{%
    \gdef\@journal{socsci}
    \gdef\@journalfull{Social Sciences}
    \gdef\@journalshort{Soc. Sci.}
    \gdef\@doiabbr{socsci}
    \gdef\@ISSN{2076-0760}
    \gdef\@societyowner{}
}
\DeclareOption{software}{%
    \gdef\@journal{software}
    \gdef\@journalfull{Software}
    \gdef\@journalshort{Software}
    \gdef\@doiabbr{software}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{soilsystems}{%
    \gdef\@journal{soilsystems}
    \gdef\@journalfull{Soil Systems}
    \gdef\@journalshort{Soil Syst.}
    \gdef\@doiabbr{soilsystems}
    \gdef\@ISSN{2571-8789}
    \gdef\@societyowner{}
}
\DeclareOption{solar}{%
    \gdef\@journal{solar}
    \gdef\@journalfull{Solar}
    \gdef\@journalshort{Solar}
    \gdef\@doiabbr{solar}
    \gdef\@ISSN{2673-9941}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{solids}{%
    \gdef\@journal{solids}
    \gdef\@journalfull{Solids}
    \gdef\@journalshort{Solids}
    \gdef\@doiabbr{solids}
    \gdef\@ISSN{2673-6497}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{spectroscj}{%
    \gdef\@journal{spectroscj}
    \gdef\@journalfull{Spectroscopy Journal}
    \gdef\@journalshort{Spectrosc. J.}
    \gdef\@doiabbr{spectroscj}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{sports}{%
    \gdef\@journal{sports}
    \gdef\@journalfull{Sports}
    \gdef\@journalshort{Sports}
    \gdef\@doiabbr{sports}
    \gdef\@ISSN{2075-4663}
    \gdef\@societyowner{}
}
\DeclareOption{standards}{%
    \gdef\@journal{standards}
    \gdef\@journalfull{Standards}
    \gdef\@journalshort{Standards}
    \gdef\@doiabbr{standards}
    \gdef\@ISSN{2305-6703}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{stats}{%
    \gdef\@journal{stats}
    \gdef\@journalfull{Stats}
    \gdef\@journalshort{Stats}
    \gdef\@doiabbr{stats}
    \gdef\@ISSN{2571-905X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{std}{%
    \gdef\@journal{std}
    \gdef\@journalfull{Surgical Techniques Development}
    \gdef\@journalshort{Surg. Tech. Dev.}
    \gdef\@doiabbr{std}
    \gdef\@ISSN{2038-9582}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{stresses}{%
    \gdef\@journal{stresses}
    \gdef\@journalfull{Stresses}
    \gdef\@journalshort{Stresses}
    \gdef\@doiabbr{stresses}
    \gdef\@ISSN{2673-7140}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{surfaces}{%
    \gdef\@journal{surfaces}
    \gdef\@journalfull{Surfaces}
    \gdef\@journalshort{Surfaces}
    \gdef\@doiabbr{surfaces}
    \gdef\@ISSN{2571-9637}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{surgeries}{%
    \gdef\@journal{surgeries}
    \gdef\@journalfull{Surgeries}
    \gdef\@journalshort{Surgeries}
    \gdef\@doiabbr{surgeries}
    \gdef\@ISSN{2017-2017}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{suschem}{%
    \gdef\@journal{suschem}
    \gdef\@journalfull{Sustainable Chemistry}
    \gdef\@journalshort{Sustain. Chem.}
    \gdef\@doiabbr{suschem}
    \gdef\@ISSN{2673-4079}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{sustainability}{%
    \gdef\@journal{sustainability}
    \gdef\@journalfull{Sustainability}
    \gdef\@journalshort{Sustainability}
    \gdef\@doiabbr{su}
    \gdef\@ISSN{2071-1050}
    \gdef\@societyowner{}
}
\DeclareOption{symmetry}{%
    \gdef\@journal{symmetry}
    \gdef\@journalfull{Symmetry}
    \gdef\@journalshort{Symmetry}
    \gdef\@doiabbr{sym}
    \gdef\@ISSN{2073-8994}
    \gdef\@societyowner{}
}
\DeclareOption{synbio}{%
    \gdef\@journal{synbio}
    \gdef\@journalfull{SynBio}
    \gdef\@journalshort{SynBio}
    \gdef\@doiabbr{synbio}
    \gdef\@ISSN{2674-0583}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{systems}{%
    \gdef\@journal{systems}
    \gdef\@journalfull{Systems}
    \gdef\@journalshort{Systems}
    \gdef\@doiabbr{systems}
    \gdef\@ISSN{2079-8954}
    \gdef\@societyowner{}
}
\DeclareOption{targets}{%
    \gdef\@journal{targets}
    \gdef\@journalfull{Targets}
    \gdef\@journalshort{Targets}
    \gdef\@doiabbr{targets}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{taxonomy}{%
    \gdef\@journal{taxonomy}
    \gdef\@journalfull{Taxonomy}
    \gdef\@journalshort{Taxonomy}
    \gdef\@doiabbr{taxonomy}
    \gdef\@ISSN{2673-6500}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{technologies}{%
    \gdef\@journal{technologies}
    \gdef\@journalfull{Technologies}
    \gdef\@journalshort{Technologies}
    \gdef\@doiabbr{technologies}
    \gdef\@ISSN{2227-7080}
    \gdef\@societyowner{}
}
\DeclareOption{telecom}{%
    \gdef\@journal{telecom}
    \gdef\@journalfull{Telecom}
    \gdef\@journalshort{Telecom}
    \gdef\@doiabbr{telecom}
    \gdef\@ISSN{2673-4001}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{test}{%
    \gdef\@journal{test}
    \gdef\@journalfull{Test}
    \gdef\@journalshort{Test}
    \gdef\@doiabbr{}
    \gdef\@ISSN{}
    \gdef\@societyowner{}
}
\DeclareOption{textiles}{%
    \gdef\@journal{textiles}
    \gdef\@journalfull{Textiles}
    \gdef\@journalshort{Textiles}
    \gdef\@doiabbr{textiles}
    \gdef\@ISSN{2673-7248}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{thalassrep}{%
    \gdef\@journal{thalassrep}
    \gdef\@journalfull{Thalassemia Reports}
    \gdef\@journalshort{Thalass. Rep.}
    \gdef\@doiabbr{thalassrep}
    \gdef\@ISSN{2039-4365}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{therapeutics}{%
    \gdef\@journal{therapeutics}
    \gdef\@journalfull{Therapeutics}
    \gdef\@journalshort{Therapeutics}
    \gdef\@doiabbr{therapeutics}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{thermo}{%
    \gdef\@journal{thermo}
    \gdef\@journalfull{Thermo}
    \gdef\@journalshort{Thermo}
    \gdef\@doiabbr{thermo}
    \gdef\@ISSN{2673-7264}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{timespace}{%
    \gdef\@journal{timespace}
    \gdef\@journalfull{Time and Space}
    \gdef\@journalshort{Time Space}
    \gdef\@doiabbr{timespace}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{tomography}{%
    \gdef\@journal{tomography}
    \gdef\@journalfull{Tomography}
    \gdef\@journalshort{Tomography}
    \gdef\@doiabbr{tomography}
    \gdef\@ISSN{2379-139X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{tourismhosp}{%
    \gdef\@journal{tourismhosp}
    \gdef\@journalfull{Tourism and Hospitality}
    \gdef\@journalshort{Tour. Hosp.}
    \gdef\@doiabbr{tourhosp}
    \gdef\@ISSN{2673-5768}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{toxics}{%
    \gdef\@journal{toxics}
    \gdef\@journalfull{Toxics}
    \gdef\@journalshort{Toxics}
    \gdef\@doiabbr{toxics}
    \gdef\@ISSN{2305-6304}
    \gdef\@societyowner{}
}
\DeclareOption{toxins}{%
    \gdef\@journal{toxins}
    \gdef\@journalfull{Toxins}
    \gdef\@journalshort{Toxins}
    \gdef\@doiabbr{toxins}
    \gdef\@ISSN{2072-6651}
    \gdef\@societyowner{}
}
\DeclareOption{transplantology}{%
    \gdef\@journal{transplantology}
    \gdef\@journalfull{Transplantology}
    \gdef\@journalshort{Transplantology}
    \gdef\@doiabbr{transplantology}
    \gdef\@ISSN{2673-3943}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{transportation}{%
    \gdef\@journal{transportation}
    \gdef\@journalfull{Transportation}
    \gdef\@journalshort{Transportation}
    \gdef\@doiabbr{transportation}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{traumacare}{%
    \gdef\@journal{traumacare}
    \gdef\@journalfull{Trauma Care}
    \gdef\@journalshort{Trauma Care}
    \gdef\@doiabbr{traumacare}
    \gdef\@ISSN{2673-866X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{traumas}{%
    \gdef\@journal{traumas}
    \gdef\@journalfull{Traumas}
    \gdef\@journalshort{Traumas}
    \gdef\@doiabbr{traumas}
    \gdef\@ISSN{2673-7477}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{tropicalmed}{%
    \gdef\@journal{tropicalmed}
    \gdef\@journalfull{Tropical Medicine and Infectious Disease}
    \gdef\@journalshort{Trop. Med. Infect. Dis.}
    \gdef\@doiabbr{tropicalmed}
    \gdef\@ISSN{2414-6366}
    \gdef\@societyowner{}
}
\DeclareOption{universe}{%
    \gdef\@journal{universe}
    \gdef\@journalfull{Universe}
    \gdef\@journalshort{Universe}
    \gdef\@doiabbr{universe}
    \gdef\@ISSN{2218-1997}
    \gdef\@societyowner{}
}
\DeclareOption{urbansci}{%
    \gdef\@journal{urbansci}
    \gdef\@journalfull{Urban Science}
    \gdef\@journalshort{Urban Sci.}
    \gdef\@doiabbr{urbansci}
    \gdef\@ISSN{2413-8851}
    \gdef\@societyowner{}
}
\DeclareOption{uro}{%
    \gdef\@journal{uro}
    \gdef\@journalfull{Uro}
    \gdef\@journalshort{Uro}
    \gdef\@doiabbr{uro}
    \gdef\@ISSN{2673-4397}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{vaccines}{%
    \gdef\@journal{vaccines}
    \gdef\@journalfull{Vaccines}
    \gdef\@journalshort{Vaccines}
    \gdef\@doiabbr{vaccines}
    \gdef\@ISSN{2076-393X}
    \gdef\@societyowner{}
}
\DeclareOption{vehicles}{%
    \gdef\@journal{vehicles}
    \gdef\@journalfull{Vehicles}
    \gdef\@journalshort{Vehicles}
    \gdef\@doiabbr{vehicles}
    \gdef\@ISSN{2624-8921}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{venereology}{%
    \gdef\@journal{venereology}
    \gdef\@journalfull{Venereology}
    \gdef\@journalshort{Venereology}
    \gdef\@doiabbr{venereology}
    \gdef\@ISSN{2674-0710}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{vetsci}{%
    \gdef\@journal{vetsci}
    \gdef\@journalfull{Veterinary Sciences}
    \gdef\@journalshort{Vet. Sci.}
    \gdef\@doiabbr{vetsci}
    \gdef\@ISSN{2306-7381}
    \gdef\@societyowner{}
}
\DeclareOption{vibration}{%
    \gdef\@journal{vibration}
    \gdef\@journalfull{Vibration}
    \gdef\@journalshort{Vibration}
    \gdef\@doiabbr{vibration}
    \gdef\@ISSN{2571-631X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{virtualworlds}{%
    \gdef\@journal{virtualworlds}
    \gdef\@journalfull{Virtual Worlds}
    \gdef\@journalshort{Virtual Worlds}
    \gdef\@doiabbr{virtualworlds}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{viruses}{%
    \gdef\@journal{viruses}
    \gdef\@journalfull{Viruses}
    \gdef\@journalshort{Viruses}
    \gdef\@doiabbr{v}
    \gdef\@ISSN{1999-4915}
    \gdef\@societyowner{}
}
\DeclareOption{vision}{%
    \gdef\@journal{vision}
    \gdef\@journalfull{Vision}
    \gdef\@journalshort{Vision}
    \gdef\@doiabbr{vision}
    \gdef\@ISSN{2411-5150}
    \gdef\@societyowner{}
}
\DeclareOption{waste}{%
    \gdef\@journal{waste}
    \gdef\@journalfull{Waste}
    \gdef\@journalshort{Waste}
    \gdef\@doiabbr{waste}
    \gdef\@ISSN{2813-0391}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{water}{%
    \gdef\@journal{water}
    \gdef\@journalfull{Water}
    \gdef\@journalshort{Water}
    \gdef\@doiabbr{w}
    \gdef\@ISSN{2073-4441}
    \gdef\@societyowner{}
}
\DeclareOption{wem}{%
    \gdef\@journal{wem}
    \gdef\@journalfull{Wildlife Ecology and Management}
    \gdef\@journalshort{Wildl. Ecol. Manag.}
    \gdef\@doiabbr{}
    \gdef\@ISSN{1234-4321}
    \gdef\@societyowner{}
}
\DeclareOption{wevj}{%
    \gdef\@journal{wevj}
    \gdef\@journalfull{World Electric Vehicle Journal}
    \gdef\@journalshort{World Electr. Veh. J.}
    \gdef\@doiabbr{wevj}
    \gdef\@ISSN{2032-6653}
    \gdef\@societyowner{World Electric Vehicle Association}
}
\DeclareOption{wild}{%
    \gdef\@journal{wild}
    \gdef\@journalfull{Wild}
    \gdef\@journalshort{Wild}
    \gdef\@doiabbr{wild}
    \gdef\@ISSN{}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{wind}{%
    \gdef\@journal{wind}
    \gdef\@journalfull{Wind}
    \gdef\@journalshort{Wind}
    \gdef\@doiabbr{wind}
    \gdef\@ISSN{2674-032X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{women}{%
    \gdef\@journal{women}
    \gdef\@journalfull{Women}
    \gdef\@journalshort{Women}
    \gdef\@doiabbr{women}
    \gdef\@ISSN{2673-4184}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{world}{%
    \gdef\@journal{world}
    \gdef\@journalfull{World}
    \gdef\@journalshort{World}
    \gdef\@doiabbr{world}
    \gdef\@ISSN{2673-4060}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{youth}{%
    \gdef\@journal{youth}
    \gdef\@journalfull{Youth}
    \gdef\@journalshort{Youth}
    \gdef\@doiabbr{youth}
    \gdef\@ISSN{2673-995X}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}
\DeclareOption{zoonoticdis}{%
    \gdef\@journal{zoonoticdis}
    \gdef\@journalfull{Zoonotic Diseases}
    \gdef\@journalshort{Zoonotic Dis.}
    \gdef\@doiabbr{zoonoticdis}
    \gdef\@ISSN{2813-0227}
    \gdef\@continuouspages{yes}
    \gdef\@societyowner{}
}

